On the amplification of security and privacy risks by post-hoc explanations in machine learning models

A variety of explanation methods have been proposed in recent years to help users gain insights into the results returned by neural networks, which are otherwise complex and opaque black-boxes. However, explanations give rise to potential side-channels that can be leveraged by an adversary for mounting attacks on the system. In particular, post-hoc explanation methods that highlight input dimensions according to their importance or relevance to the result also leak information that weakens security and privacy. In this work, we perform the first systematic characterization of the privacy and security risks arising from various popular explanation techniques. First, we propose novel explanation-guided black-box evasion attacks that lead to 10 times reduction in query count for the same success rate. We show that the adversarial advantage from explanations can be quantified as a reduction in the total variance of the estimated gradient. Second, we revisit the membership information leaked by common explanations. Contrary to observations in prior studies, via our modified attacks we show significant leakage of membership information (above 100% improvement over prior results), even in a much stricter black-box setting. Finally, we study explanation-guided model extraction attacks and demonstrate adversarial gains through a large reduction in query count.

==> TIFS-2022 (Arxiv) 2/E.tex <==
\section{Evasion Attacks (EA)}
\label{sec:problem}
%\subsection{Threat model for producing adversarial perturbation}
\begin{table}[]
\begin{adjustbox}{max width=0.45\textwidth}
    \begin{tabular}{l|l}
    \hline
    Notation & Definition\\ 
    \hline
    ${\bf x}$ & Input to the model\\
    \hline
    ${F(\bf x)}_i$ & Logit score of the $i$-th class\\
    \hline
    $f(\bf x)=\boldsymbol{\sigma}(F(\bf x))$ & Softmax scores of the output logit \\
    \hline
    $\nabla_{\mathbf x} f(\mathbf x)_i$ & Gradient of the softmax score of the $i$-th class w.r.t input\\
    \hline
    $E(F, \bf x)$ & Explanation in the input space produced by the logit\\ 
    \hline
    $E(f, \bf x)$ & Explanation produced by the softmax score\\ 
    \hline
    $\boldsymbol{e}$ & An instance produced by $E$ (true explanation)\\ 
    \hline
    % $|\boldsymbol{e}|$ & Element-wise absolute value of $\boldsymbol{e}$ 
    % (absolute-value explanation)\\ 
    $|\boldsymbol{e}|$ & \makecell{Element-wise absolute value of $\boldsymbol{e}$ \\
    (absolute-value explanation)}\\ 
    \hline
    \end{tabular}
\end{adjustbox}
\caption{Summary of notations used in the paper}\label{table:notations}
\vspace{-2em}
\end{table}

{\bf Notation:} Let ${\bf x} \in \mathbb{R}^n$ be the input and ${\bf x}_{adv} \in \mathbb{R}^n$ be the corresponding adversarial example that we want to generate. We denote the victim model as $F(\bf{x}): \mathbb{R}^n \rightarrow \mathbb{R}^k$ where $k$ is the number of classes and $f(\bf x)$ is the corresponding probability for each class. Let $\nabla_{\mathbf x} f(\mathbf x)_i \in \mathbb{R}^{n}$ be the gradient of the output probability (softmax score) w.r.t the input for the $i-$th label. We denote by $E: \mathbb{R}^{n} \rightarrow \mathbb{R}^n$ the class of explanation mechanisms, that take gradient vector for an output label as input and generates a saliency map as the output. The saliency map is the same size as the input. Table. \ref{table:notations} summarizes the common notations used.

\noindent{\bf Adversary Access:} In most practical settings, adversarial examples must be considered under a limited threat model which prompted us to study black-box attacks, where the adversary only has query-access to the target model~\cite{ilyas2018black}. 
%\noindent {\bf Adversary Access:} 
In this setting, an adversary provides a query input $\mathbf x$ to the model and can only observe the model's response to the query. Specifically, the response consists of the output of the explanation mechanism in addition to the output of the victim model. The adversary does not have access to the model weights and cannot directly compute the gradient w.r.t the model parameters.

\subsection{Background}
We consider $l_2$-norm bounded perturbation of the input with the goal of performing both targeted (i.e., misclassification to a given target class) and untargeted (i.e., misclassification to any class other than the true class) attacks. Based on additional constraints on the model response in the black-box setting, we consider attacks under the following two threat models:

\subsubsection{Soft-label attack} 
In this setting, the adversary has access to the predicted probabilities over all or the top-k classes. Prior work have used the information to generate adversarial inputs via zeroth-order optimization methods (e.g., finite-difference method)~\cite{chen2017zoo, ilyas2018black} and gradient-free techniques (e.g., genetic algorithm)~\cite{alzantot2019genattack}. Here an adversary has access to the predicted class $t$, as well as the prediction probability vector $f({\bf x})_y$ for all classes $y$. We define a loss function $\mathcal{L}({\mathbf x})$ as $\mathcal{L}(\mathbf{x}) = f(\mathbf{x})_t\mathbf{1}_{\{f(\mathbf{x})_t>\underset{i\neq t}{\mathrm{max}}\text{ }f(\mathbf{x})_i \}}$.
% \begin{equation}
%     \mathcal{L}(\mathbf{x}) = f(\mathbf{x})_t\mathbf{1}_{\{f(\mathbf{x})_t>\underset{i\neq t}{\mathrm{max}}\text{ }f(\mathbf{x})_i \}}
% \end{equation}
Our objective in this setting is to perform an untargeted attack. Note, $\mathcal{L}({\mathbf x})=0$ only when the predicted class does not equal the target class $t$. The attack can thus be formulated as $\mathbf{x}_{adv} = \underset{\mathbf{z}: ||\mathbf{x}-\mathbf{z}||_2\leq \epsilon}{\mathrm{arg\,min}} \mathcal{L}(\mathbf{z})$, where $\epsilon$ is the perturbation budget.
% \begin{equation}
% \label{eqn:soft_label_obj}
%      \mathbf{x}_{adv} = \underset{\mathbf{z}: ||\mathbf{x}-\mathbf{z}||_2\leq \epsilon}{\mathrm{arg\,min}} \mathcal{L}(\mathbf{z})
% \end{equation}
The above objective can be optimized by taking a step in the direction of the gradient of the loss followed by a projection onto the feasible set. We follow the modified NES gradient-free approach~\cite{wierstra2014natural} to estimate the gradient of $f(\mathbf{x})$ as:
\begin{equation}\label{nes}
    \widetilde{\nabla f(\mathbf{x})} = \frac{1}{2\delta B} \sum_{b=1}^B (f(\mathbf{x}+\delta\mathbf{u}_b)_i-f(\mathbf{x}-\delta\mathbf{u}_b)_i )\mathbf{u}_b 
\end{equation}
where $\delta$ is the perturbation parameter, $\mathbf{u}_b \in \mathbb{R}^n$, and $\{\mathbf{u}_b\}_{b=1}^{B}$ are i.i.d. samples from the normal distribution $\mathcal N(\mathbf{0}, \epsilon\mathbf{I})$, in a manner similar to \cite{wierstra2014natural, ilyas2018black}. Given the estimated gradient, the adversarial inputs are generated via an approach similar to PGD~\cite{madry2017towards}.

\subsubsection{Hard-label attack}
In this setting, only the top-1 predicted label is output by the model ~\cite{chen2020hopskipjumpattack, cheng2019sign}. The resulting discontinuous and combinatorial attack problem is first transformed into a random-walk problem along the decision boundary in~\cite{chen2020hopskipjumpattack}. Below we summarize the formulation of the hard-label attack for generating an adversarial example as proposed in~\cite{chen2020hopskipjumpattack}.
%formalize the hard-label attack for generating an adversarial example proposed in~\cite{chen2020hopskipjumpattack}. 
We define a decision function $\phi_t(\mathbf{x})$ as:
%Similarly, the decision function of hard-label attack $\phi_t(\mathbf{x})$ can be defined as:
\begin{equation}\label{M}
	\begin{aligned}
	& &\phi_t(\mathbf{x}) \overset{def}{:=} \left\{\begin{array}{ll}
	1, & \text{if prediction is in the target class } t\\
	-1, &  \text{otherwise}\\
	\end{array}
	\right.\\
	\\
	\end{aligned}
\end{equation}
A decision attack objective can then be formulated as $\mathbf{x}_{adv} = \underset{\mathbf{z}: \phi_t(\mathbf{z})=1}{\mathrm{arg\,min}}||\mathbf{x}-\mathbf{z}||$.
% \begin{equation}
% \label{eqn:hard_label_obj}
%     \mathbf{x}_{adv} = \underset{\mathbf{z}: \phi_t(\mathbf{z})=1}{\mathrm{arg\,min}}||\mathbf{x}-\mathbf{z}||
% \end{equation}
%The optimization of the above objective via a random walk along the decision boundary $\phi_t(\mathbf{x})=1$ is proposed in~\cite{chen2020hopskipjumpattack}.
The goal is to minimize the distance of the adversarial sample to $\bf x$ while satisfying the boundary constraint $\phi_t(\mathbf{x})=1$. This is performed via a random walk along the decision boundary, in which the direction of the next step is estimated using the gradient of $\phi_t(\mathbf{x})$ as:
\begin{equation}\label{hsja}
    \widetilde{\nabla \phi_t}(\mathbf{x}) = \frac{1}{B}\sum_{b=1}^B \phi_t(\mathbf{x}+\delta \mathbf{u}_b) \mathbf{u}_b
\end{equation}

where $\delta$ is the perturbation parameter, $\mathbf{u}_b \in \mathbb{R}^n$, and $\{\mathbf{u}_b\}_{b=1}^{B}$ are i.i.d. samples from the normal distribution $\mathcal N(\mathbf{0}, \epsilon\mathbf{I})$.

% \begin{itemize}
% \item Soft-label attack: In this setting, the adversary has access to the predicted probabilities over all or the top-k classes. Prior work have used the information to generate adversarial inputs via zeroth-order optimization methods (e.g., finite-difference method)~\cite{chen2017zoo, ilyas2018black} and gradient-free techniques (e.g., genetic algorithm)~\cite{alzantot2019genattack}.

% \item Hard-label attack: In this setting, only the top-1 predicted label is output by the model. In ~\cite{brendel2017decision, chen2020hopskipjumpattack} the authors propose random walks along the decision boundary to produce adversarial inputs. \cite{cheng2019sign, cheng2018query} first transformed the discontinuous and combinatorial problem into a real-valued optimization problem and then applied standard zeroth-order optimization algorithm.
% \end{itemize}

% We assume that in addition to the victim model's decision, the explanation is also available to the adversary. Our goal is to perform a query-efficient attack using explanation as an addition source of information.

\subsection{Our Attack Strategies for EA}
\label{sec:strategies}
%One of the widely used explanation is feature-based saliency map, where elements responsible for model decision are highlighted \cite{simonyan2013deep, sundararajan2017axiomatic, smilkov2017smoothgrad}. Typically, people usually return $\mathbf{E}(\mathbf{x}; \mathbf{F}) \in [0, 1]^N$ for visualization where the absolute value of gradients is kept. The strategy is found more clearly explaining the model's decision of images as observed in \cite{simonyan2013deep, smilkov2017smoothgrad}.
Generating adversarial examples in the black-box setting requires an adversary to estimate the model gradient. Rather than optimizing for a specific attack objective 
%as specified in the previous discussions, 
prior work have explored the idea of a \emph{search distribution} and have established that an adversary can maximize the expected value of the attack objective, under the search distribution, using far fewer number of queries~\cite{ilyas2018black}.

In our attacks we adopt this idea of sampling from a suitable search distribution to estimate the gradient vector. We propose three different attacks, each designed to exploit the information in model explanation in different ways. The attacks are applicable for soft-label and hard-label settings and can be used for both targeted, and untargeted misclassification.

% We provide a taxonomy of the attacks identifying the conditions under which they perform the best in Fig.\ref{fig:conditions}:
% %We explain the attacks in detail below as shown in Fig. \ref{fig:conditions}: 
% (\romannumeral 1) If the true explanation is available, the attacker can use EGTA when the explanation is similar to the gradient; (\romannumeral 2) If the true explanation is available but the form is different from the true gradient, the attacker can use EGSMA. (\romannumeral 3) If only the absolute-value explanation is accessible, the attacker can use EGSA. 
% By inspecting the returned explanations, the attacker can know which form of the explanation is used so he can apply different strategies accordingly.}

% \begin{figure}[h]
% \includegraphics[width=0.98\linewidth]{images/ATK-flow.png}  \centering
% 	\caption{The attack strategy can be used in different conditions.}
% 	\label{fig:conditions}
% \end{figure}

\begin{figure}[h]
\includegraphics[width=0.98\linewidth]{images/EGTA.png}  \centering
	\caption{Explanation-Guided Transfer Attack  (EGTA)}
	\label{fig:egta}
\end{figure}
\noindent{\textbf{Explanation-guided Transfer Attack (EGTA)}} We consider an adversary that samples vectors $\mathbf{u}_b$ from a normal distribution $\mathcal N(\mathbf{0}, \epsilon \mathbf{I})$ to perform gradient estimation. If the adversary had prior knowledge that gradient ${\bf g} = \nabla_{\bf x} F({\bf x})$ is used to compute the explanation ${\bf e} = E(F, \bf{x})$ then it can use the explanation to shape the search distribution by incorporating it as a prior. Besides, we also let its norm $||\boldsymbol e||=1$. In this case, the sampled vector $\mathbf{u}_b \in \mathbb{R}^n$ for  \eqref{nes} and \eqref{hsja} can be expressed as:

\begin{equation}\label{eq:direct_transfer}
    \mathbf{u}_b = \sqrt{\lambda} \mathbf{u} + \sqrt{1-\lambda} \mathbf{e}
\end{equation}
where $\mathbf{u} \sim \mathcal N(\mathbf{0}, \epsilon\mathbf{I})$. We use $\lambda \in [0, 1]$ to reflect adversarial confidence of the prior knowledge. We adopt \eqref{eq:direct_transfer} as our attack strategy and name it as Explanation-guided Transfer Attack (EGTA) as shown in Fig. \ref{fig:egta}.


Using the transfer prior \eqref{eq:direct_transfer}, the total estimation variance equals (both total variance and bias are derived in the appendix \ref{sec:variance}):
\begin{align}\label{eqn:tv}
		\text{total variance} & = \text{tr}(\text{Var}(\widetilde{\nabla f(\mathbf{x})}) \nonumber \\
		& = \frac{1}{B}(\lambda^2(n+1)||\nabla f(\mathbf{x})||_2^2 + 4(1-\lambda)\lambda (\nabla f(\mathbf{x})^T \boldsymbol{e})^2) \nonumber
\end{align}

%Especially,

\begin{equation*}
    \text{Specifically, total variance} = \left\{\begin{array}{ll}
        \frac{n+1}{B}||\nabla f(\mathbf{x})||_2^2, & \text{when } \lambda=1\\
        % \lambda^2(n+1)||\nabla f(\mathbf{x})||_2^2 + 4(1-\lambda) (\nabla f(\mathbf{x})^T \boldsymbol{e})^2, & 0 \leq \lambda \leq 1\\
        0, & \text{when } \lambda=0
        \end{array}
        \right.
\end{equation*}

Here, $(n+1)||\nabla f(\mathbf{x})||_2^2 \gg 4 (\nabla f(\mathbf{x})^T \boldsymbol{e})^2 $ as $n$ is typically larger than 1 for high dimensional data such as images and $||\nabla f(\mathbf{x})||_2^2 \geq (\nabla f(\mathbf{x})^T \boldsymbol{e})^2$. \revisionPQ{}{Therefore, $\frac{d \text{tr}(\text{Var}(\widetilde{\nabla f(\mathbf{x})})}{d \lambda} = \frac{2}{B}(((n+1)||\nabla f(\mathbf{x})||_2^2-4(\nabla f(\mathbf{x})^T \boldsymbol{e})^2)\lambda+2(\nabla f(\mathbf{x})^T \boldsymbol{e})^2) \geq 0$ for $\forall \lambda \in [0, 1]$, which means the total variance will monotonically decrease as $\lambda$ decreases. Thus, when $\lambda$ is closer to 0, i.e., the search direction relies more on the prior explanation, the variance will be much lower than the case where no search direction is provided (i.e., setting $\lambda$ close to 1).}

Besides, the estimation $\text{bias} = (1-\lambda)^2 || \nabla f(\mathbf{x})||_2^2(1-\text{cos}(\theta)^2)$, where $\text{cos}(\theta)$ is the cosine similarity between $\boldsymbol{e}$ and $\nabla f(\mathbf{x})$. The bias will decrease as $\text{cos}(\theta)$ increases, which indicates that EGTA is useful for $\boldsymbol e$ that is similar to the gradient, i.e., has a larger cosine similarity to the gradient.

\noindent{\textbf{Explanation-guided Sampling Attack (EGSA):}} Explanations using the absolute value of the gradients may lead to cleaner visualization~\cite{simonyan2013deep, smilkov2017smoothgrad} and the explanation mechanism may return $\mathbf{|e|}$ to the users. In this case, directly using EGTA will lead to a highly biased gradient estimation. To address this we propose EGSA based on the intuition that for locations that has a small gradient value, the corresponding explanation value should also be small. Therefore, we dynamically scale the value of the search vector $\mathbf{u}$ according to the explanation value. Moreover, in appendix \ref{sec:opt_approx}, we theoretically quantify the advantage of EGSA by proving the optimality of the covariance matrix approximation step. 

EGSA can be implemented by replacing \eqref{eq:direct_transfer} with the following\footnote{$\odot$ denotes the Hadamard product.} in Fig. \ref{fig:egta}:

\begin{equation}\label{eq:transfer_sample}
    \mathbf{u}_b = \sqrt{\lambda} \mathbf{u} + \sqrt{1-\lambda} \mathbf{|e|} \odot \mathbf{u}
\end{equation}

%
%As mentioned in Section~\ref{sec:problem}, we consider saliency maps as explanations. More specifically, we consider explanation mechanisms that use the absolute value of the gradient (ignoring their signs) as the explanation~\cite{simonyan2013deep, smilkov2017smoothgrad}. Thus, in our setting, the explanation $\mathbf E$ instead of $\mathbf g$ is available. In other words, we assume $E_i$ is equivalent to $|g_i|$ and not $g_i$.
%Therefore, setting $\mathbf{E}$ as the transfer prior $\mathbf{g}$ and using the covariance matrix in Eqn.~\eqref{eqn: sigma} will lead to noisy estimation of the gradient as $\mathbb{E}[u_{b,i},u_{b,j}]=E_i E_j = |g_i g_j| \neq g_i g_j$ for $i\neq j$. 
%
%Note that the diagonal of the covariance matrix $\mathbf{\Sigma}$, $E_i E_j = g_i g_j$ if $\mathbf{E}$ is set as the transfer prior in Eqn. \eqref{eqn: sigma}. We therefore design the covariance matrix of the search distribution as follows:
%
%\begin{equation}\label{eq:transfer}
%    \mathbf{\Sigma^*} = \lambda \epsilon \mathbf{I} + (1-\lambda) \text{diag}(\mathbf{E}\odot\mathbf{E})
%\end{equation}

% Note that $\sigma_{ij}$ is the element in the $i$-th row and $j$-th column of the matrix $\mathbf{\Sigma}$. In appendix \ref{sec:opt_approx}, we show that $\mathbf{\Sigma^*}$ is the minimizer of the \textit{KL divergence} between the distribution $\mathcal N(\mathbf{0}, \mathbf{\Sigma})$ and the distribution $\mathcal N(\mathbf{0}, \mathbf{\Sigma'})$ for any $\mathbf{\Sigma'} \in \mathbb{D}=  \{\text{diag}(\sigma_{11},...\sigma_{NN}) | \sigma_{ii} \geq 0 \text{ for }\forall i \in [1,...,N]\}$. 


\noindent{\textbf{Explanation-Guided Surrogate Model Attack (EGSMA)}} Given an input $\mathbf x$, the black-box model $f(\mathbf x)$, and  explanation $E$, we fine tune a surrogate model $\tilde{f}(\mathbf x)$ for efficient attacks as shown in Fig. \ref{fig:egsma}. In this attack, we assume that the adversary knows the explanation mechanism that is being used by the victim model to generate the explanation. 

\begin{figure}[h]
\includegraphics[width=0.9\linewidth]{images/EGSMA.png}  \centering
	\caption{Explanation-Guided  Surrogate  Model  Attack  (EGSMA)}
	\label{fig:egsma}
	\vspace{-1em}
\end{figure}
We train the surrogate model such that for a given input its prediction matches that of the victim model. To perform training, we use the information available from both the victim model as well as the explanation as follows.

Let $t$ be the label predicted by the victim model. We define the prediction loss of the surrogate model $\mathcal{L}_{pred}\overset{def}{:=}\tilde{f}_t(\mathbf x) - \underset{i\neq t}{\mathrm{max}}\text{ } \tilde{f}_i(\mathbf x)$. Thus, the surrogate model is penalized only when the logit score of the predicted class $t$ denoted by $\tilde{f}_t$, is not the largest among all classes. This will cause the surrogate model to mimic the prediction of the victim model. In addition, we also force the explanation provided by the surrogate model to be close to the true explanation by minimizing $\mathcal{L}_{expln}\overset{def}{:=}||{\mathbf e}-\mathbf{\tilde{e}}||$. Here ${\mathbf e}$ is produced by the victim model and $\tilde{\mathbf e}$ is generated using the gradient vector from the surrogate model. 

We combine the prediction and explanation losses to train the surrogate model using $\mathcal{L}_{sur}$ loss defined as:
\begin{equation}\label{eqn:egsma_loss}
    \mathcal{L}_{sur} = \mathcal{L}_{pred} + \alpha \mathcal{L}_{expln}
\end{equation}

After fine tuning the surrogate model on the loss Eqn.~\eqref{eqn:egsma_loss} with $\alpha \in [0, 1]$, we use EGSA to find the adversarial example.

\begin{figure}[h]
\includegraphics[width=0.98\linewidth]{images/ATK-flow.png}  \centering
	\caption{Choosing the attack strategy based on explanation type}
	\label{fig:conditions}
\end{figure}

\noindent{{\bf Choosing the best attack strategy:}}
\revisionPQ{}{We provide a taxonomy of the attacks identifying the conditions under which they perform the best in Fig.\ref{fig:conditions}. For distinction, we call $\boldsymbol{e}$, which is directly produced from explanation mechanism, as a \textit{true explanation}, and $|\boldsymbol{e}|$ as the \textit{absolute-value explanation} as shown in Table \ref{table:notations}}. (\romannumeral 1) If the true explanation is available, the attacker can use EGTA when the explanation is similar to the gradient; (\romannumeral 2) If the true explanation is available but the form is different from the true gradient, the attacker can use EGSMA. (\romannumeral 3) If only the absolute-value explanation is accessible, the attacker can use EGSA. 
By inspecting the returned explanations, the attacker can know which form of the explanation is used so he can choose the attack strategy based on the explanation type.



==> TIFS-2022 (Arxiv) 2/ME.tex <==
\section{Model Extraction attack (MEA)}
% {\bf Background:} Despite the fact that machine learning and neural networks are widely applied in industry settings, the trained models are costly to obtain. Furthermore, there are security \cite{carlini2017towards, carlini2017adversarial} and privacy \cite{shokri2017membership, fredrikson2015model} concerns for revealing trained models to potential adversaries. Therefore, the trained model should be treated as proprietary and need to be protected. Unfortunately, prior works \cite{tramer2016stealing, orekondy2019knockoff, oh2019towards, pal2019framework, milli2019model} have shown that an adversary with query access to a model can steal the model to obtain a copy that is \revisionPQ{}{\textit{functionally equivalent}, i.e., predictions are identical to those of the victim model on all possible inputs.} Especially, \cite{milli2019model} shows that gradient matching is a useful method to improve MEA. However, it lacks systematic study of how various explanation functions \cite{simonyan2013deep, sundararajan2017axiomatic, ribeiro2016should} can help MEA.

Despite the fact that machine learning and neural networks are widely applied in industry settings, the trained models are costly to obtain. Furthermore, there are security \cite{carlini2017towards, carlini2017adversarial} and privacy \cite{shokri2017membership, fredrikson2015model} concerns for revealing trained models to potential adversaries. Thus, trained model should be treated as proprietary and protected the same way. Unfortunately, prior works \cite{tramer2016stealing, orekondy2019knockoff, milli2019model} have shown that an adversary with query access to a model can steal the model to obtain a copy that is \revisionPQ{}{\textit{functionally equivalent}, i.e., predictions are identical to those of the victim model on all possible inputs.} In particular, \cite{milli2019model} propose gradient matching to improve MEA. However, there is no systematic study regarding how various explanations \cite{simonyan2013deep, sundararajan2017axiomatic, ribeiro2016should} can help mount MEA.

\noindent{\bf Notation:} Let ${\bf x} \in \mathbb{R}^n$ be the input, $F(\boldsymbol x)$ denote the victim model and $\hat{F}(\boldsymbol x)$ represent the extracted model.

\noindent {\bf Adversary Access:} Model extraction attacks target the confidentiality of a victim model deployed on a remote server. We assume the adversary knows the architecture of the victim model but the corresponding parameter values are unknown. We also assume that the attacker possess a subset of the training data $\mathcal{S}_{train}$. However, the adversary does not necessarily have the ground-truth labels and can query $F(\boldsymbol x)$ for obtaining the labels. Through black-box query access to the victim model $F(\boldsymbol x)$ and the corresponding explanation $E(\boldsymbol x)$, the attacker aims at producing a \textit{functionally equivalent} model: the extracted model achieves same performance on the same test dataset $\mathcal{S}_{test}$, i.e., $\forall \boldsymbol x \in \mathcal{S}_{test}$, $\hat{F}(\boldsymbol x) = F(\boldsymbol x)$.

\subsection{Our Attack: Explanation-matching Strategy}
Here we follow the strategy proposed in~\cite{milli2019model} to match the predictions and the explanations produced by the victim model $F(\boldsymbol x)$. We denote the extracted model by the adversary as $\hat{F}(\boldsymbol x)$ and the corresponding explanation as $E(\boldsymbol x)$. The adversary can perform MEA by minimizing the prediction loss, $\mathcal{L}_{P} = ||\hat{F}(\boldsymbol x) - F(\boldsymbol x)||$, and an explanation matching loss, $\mathcal{L}_{E} = ||\hat{E}(\boldsymbol x) - E(\boldsymbol x)||$. In our experiments, we minimized $\mathcal{L}_{J} = \mathcal{L}_{P} +  \alpha \mathcal{L}_{E}$ where $\alpha \in [0, 1]$. For LIME, we perform prediction matching with the interpretable model.

==> TIFS-2022 (Arxiv) 2/MI.tex <==
\section{Membership Inference Attack (MIA)}
 In this attack, the goal of an adversary is to determine if a given data sample was used to train an ML model. Successful membership inference attacks can compromise user's privacy. For instance, if a machine learning model is trained on the data collected from people with certain characteristics, by knowing that a victim’s data sample belongs to the training data of the model, the attacker can immediately learn sensitive information about the victim~\cite{shokri2017membership, sablayrolles2019white}. 

% \noindent{\bf Background:} In this setting, the adversary targets at determining whether a data item (also referred to as a data point) was used to train an ML model or not. Successful membership inference attacks can compromise user's privacy. For instance, if a machine learning model is trained on the data collected from people with certain characteristics, by knowing that a victim’s data belong to the training data of the model, the attacker can immediately learn about the characteristics of victim's status. \cite{shokri2017membership, pyrgelis2017knock, hayes2019logan, sablayrolles2019white}. 

% Among them, \cite{sablayrolles2019white} further shows that their attack \textit{MALT} is optimal given an optimal threshold under some assumptions. Besides, \cite{choquette2021label, yeom2018privacy} demonstrate that it is still feasible to perform MIA only given the predicted class label. \cite{yeom2018privacy} predicts any misclassified data point as a non-member of the training set, serving a baseline of label-only MIA. This is named as \textit{GAP-attack} Furthermore, \cite{choquette2021label} use the distance to the decision boundary geometry as an indication of individual membership. We named this attack as \textit{Boundary-attack}. However, this approach needs excessive queries of the black-box victim model to either generate adversarial example or estimate the distances. Besides, the aforementioned attacks have the limitations where they either require probability prediction of each class or the ground-truth label. \cite{shokri2021privacy} shows that it is possible to extract information of the membership from the logit-score based explanation, and we named this as \textit{OPT-var}. In this paper, we demonstrate that using the explanations MIA can be performed efficiently without having access to the prediction probability, the ground-truth label, or extensive query of the victim models. 

% \begin{table*}[]
% \begin{adjustbox}{max width=0.65\textwidth}
%     \begin{tabular}{c|c|c|c|c}
%     \toprule
%     Works             & Ground-truth label & Probability prediction & Excessive queries & Explanation \\ \midrule
%     \textit{MALT} (Sablayrolles et al. 2019 \cite{sablayrolles2019white}) &  \cmark      &      \cmark        &    \xmark       &   \xmark   \\ \midrule
%     \textit{GAP-attack} (Yeom et al. 2018 \cite{yeom2018privacy})        &     \cmark      &      \xmark        &    \xmark       &   \xmark    \\ \midrule
%     \textit{Boundary-attack} (choquette et al. 2021 \cite{choquette2021label})  &     \cmark      &      \xmark        &    \cmark       &   \xmark       \\ \midrule
%     \textit{OPT-var} (Shokri et al. 2021 \cite{shokri2021privacy})      &     \xmark      &      \xmark        &    \xmark       &   \cmark      \\ \midrule
%     Ours       &     \xmark      &      \xmark        &    \xmark       &   \cmark      \\ \bottomrule
%     \end{tabular}
% \end{adjustbox}
% \caption{The requirements for performing MIA}\label{table:requirements}
% \end{table*}

\noindent {\bf Notation:} Let ${\bf x} \in \mathbb{R}^n$ be the input, and $F(\bf x)$ denote the victim model. $\mathcal{D}_{train}$ is the dataset used to train $F(\bf x)$. $\mathcal{D}_{out}$ contains the set of $\bf x$ that are not in $\mathcal{D}_{train}$.

\noindent {\bf Adversary Access:} The attacker can provide $\bf x$ to the black-box model and obtain the prediction $F(\bf x)$ and its explanation $E(\bf x)$ in a black-box setting. Table \ref{table:requirements} summarizes the additional requirements to perform membership inference attacks for existing attack methods \cite{sablayrolles2019white, yeom2018privacy, choquette2021label, shokri2021privacy}.

\noindent {\bf Attack Objective:} Given a sample $\bf x$, the attacker aims to infer whether the sample belongs to the dataset $\mathcal{D}_{train}$ or $\mathcal{D}_{out}$.

\subsection{Our Attack: Revisiting MIA Using Explanations}
For data points that are in the training set, the victim model is certain about the prediction as the training algorithms are designed to push the points away from the decision boundary. In a white-box setting, this is indicated by a relatively low loss score on training samples, which is used to determine membership in the training data. Consequently, the gradient values computed using the loss should also be fairly small for the training samples. This intuition is used in \textit{OPT-var}~\cite{shokri2021privacy}, to mount MIA in black-box settings when explanations are available. They show that variance of the explanation $\boldsymbol{E}(F, \bf x)$ produced from the logit score $F(\bf x)$ can indicate membership.

%In other words, the model should have higher confidence on the points and the gradient values computed using the loss should be fairly small.

We build on the intuition in \textit{OPT-var}~\cite{shokri2021privacy} %and \textit{Boundary-attack}~\cite{choquette2021label}, 
but note that the logit score does not completely capture the victim model's prediction confidence.
%\textit{OPT-var} \cite{shokri2021privacy} proposed to use the variance of the explanation $\boldsymbol{E}(\bf F, \bf x)$ produced from the logit score $F(\bf x)$. 
%However, this is not the complete indication of the victim model's confidence. 
The reason is that the logit score of a particular class does not take into account the logit scores of other classes. 
%Hence, a relatively low logit gradient does not indicate the true gradient back propagated from the loss. 
\revisionPQ{}{On the other hand, the softmax function of the logit consider the interaction of classes and the corresponding gradient may contain richer membership information.} Therefore, we propose to use the variance of explanation produced from the softmax score $f(\bf x) = \boldsymbol{\sigma}(F(\bf x))$ as an indicator of membership, where $\boldsymbol{\sigma}(F(\bf x))$ is calculated as follows:
\begin{equation}
    \boldsymbol{\sigma}(F(\bf x))_i = \frac{e^{F(\bf x)_i}}{\sum_{j=1}^k{e^{F(\bf x)_j}}}
\end{equation}

The variance of explanation $\boldsymbol e=\boldsymbol{E}(\boldsymbol f, \bf x)$ is calculated as:
\begin{equation}
    \text{Var}(\boldsymbol e) = \sum_{i=1}^n (\boldsymbol{e}_i - \frac{1}{n}\sum_{j=1}^n\boldsymbol{e}_j)
\end{equation}

where $\bf{x}$ and $ \bf{e} \in \mathbb{R}^n$.

==> TIFS-2022 (Arxiv) 2/abstract.tex <==
\begin{abstract}
    A variety of explanation methods have been proposed in recent years to help users gain insights into the results returned by neural networks, which are otherwise complex and opaque black-boxes. However, explanations give rise to potential side-channels that can be leveraged by an adversary for mounting attacks on the system. In particular, \revisionPQ{}{post-hoc} explanation methods that highlight input dimensions according to their importance or relevance to the result also leak  information that weaken security and privacy. In this work, we perform the first systematic characterization of the privacy and security risks arising from various popular explanation techniques. First, we propose novel explanation-guided black-box evasion attacks that lead to $10\times$ reduction in query count for the same success rate. We show that the adversarial advantage from explanations can be quantified as a \revisionPQ{}{reduction in the total variance of the estimated gradient}. Second, we revisit the membership information leaked by common explanations. Contrary to observations in prior studies, via our modified attacks we show significant leakage of membership information (above $100\%$ improvement over prior results), even in a much stricter black-box setting. Finally, we study explanation-guided model extraction attacks and demonstrate adversarial gains through large reduction in query count. 
\end{abstract}

==> TIFS-2022 (Arxiv) 2/conclusion.tex <==
\section{Conclusion}
In this paper, we proposed several attacks that leveraged post-hoc explanations to significantly improve attack efficiency of both evasion and membership inference attacks. The improvement in model extraction attack was modest, and we empirically analyzed the  performance to be strongly connected with the mean square value of the explanation. Finally, we categorized the risk level associated with different explanations and attacks. We hope this can serve as a guide for practitioners to identify the right type of explanations depending on the sensitivity of their tasks.

% provide a summary of the information leaked, based on the improvement of attack efficiency, as an indication for practitioners to select explanations in security-and privacy-critical tasks.

==> TIFS-2022 (Arxiv) 2/defense.tex <==
\section*{EGTA: A variance reduced approach}\label{sec:variance}
In this section, we theoretically quantify the advantage of EGTA. On one hand, EGTA is a biased estimator for the true gradient. On the other hand, as it relies on the transfer prior explanation $\boldsymbol e$, it can effectively reduce the variance of the estimation. 

Let $f(\boldsymbol x)$ be the objective function, i.e., the predicted probability of the target class given by the black-box machine learning model. Let $\boldsymbol e$ be the transfer prior explanation and we also let its norm $||\boldsymbol e||=1$. Let $\mathbf{u}_b$ be the search direction and $\mathbf{u}_b = \sqrt{\lambda} \mathbf{u} + \sqrt{1-\lambda} \mathbf{e} = \hat{\mathbf{u}} + \hat{\mathbf{e}}$ and $\mathbf{u} \sim \mathcal N(\mathbf{0}, \epsilon\mathbf{I})$. Then the estimation gradient using natural evolution strategy becomes:

\begin{equation}\label{nes_suppl}
    \widetilde{\nabla f(\mathbf{x})} = \frac{1}{2\delta B} \sum_{b=1}^B (f(\mathbf{x}+\delta\mathbf{u}_b)-f(\mathbf{x}-\delta\mathbf{u}_b))\mathbf{u}_b 
\end{equation}

W.l.o.g, we assume $\delta$ and $\epsilon$ equal to 1. For the purposes of analysis, suppose $\nabla f$ exists. We can approximate the function in the local neighborhood of $\boldsymbol x$ using a second order Taylor approximation: $f(\boldsymbol x + \mathbf{u}_b) \approx f(\boldsymbol x) + \mathbf{u}_b^T\nabla f(\boldsymbol x) + \frac{1}{2}\mathbf{u}_b^T\nabla^2 f(\boldsymbol x)\mathbf{u}_b$. Substituting this expression into \eqref{nes_suppl}, we can see our estimate $\widetilde{\nabla f(\mathbf{x})}$ equal to:

\begin{equation}
    \widetilde{\nabla f(\mathbf{x})} = \frac{1}{B}\sum_{b=1}^B (\mathbf{u}_b\mathbf{u}_b^T)\nabla f(\mathbf{x})
\end{equation}

Then the expectation of $\mathbb{E}[\widetilde{\nabla f(\mathbf{x})}]$ equals:

\begin{equation}\label{eqn:mean}
    \mathbb{E}[\widetilde{\nabla f(\mathbf{x})}] = (\hat \Sigma+\hat G)\nabla f(\mathbf{x})
\end{equation}

Hence bias equals:

\begin{align}\label{eqn:bias}
		\text{bias} &= ||\mathbb{E}[\widetilde{\nabla f(\mathbf{x})}] - \nabla f(\mathbf{x})||_2^2\\
		  & = (1-\lambda)^2 \nabla f(\mathbf{x})^T(I-\boldsymbol{e} \boldsymbol{e}^T)^2\nabla f(\mathbf{x}) \\
		  & = (1-\lambda)^2(|| \nabla f(\mathbf{x})||_2^2 - ( \nabla f(\mathbf{x})^T\boldsymbol{e})^2) \\
		  & = (1-\lambda)^2 || \nabla f(\mathbf{x})||_2^2(1-\text{cos}(\theta)^2)
\end{align}

where $\text{cos}(\theta)$ is the cosine similarity between $\boldsymbol{e}$ and $\nabla f(\mathbf{x})$. When cosine similarity is high, the bias of the estimation is low.

Next we use the total variance, i.e., $\text{tr}(\text{Var}(\widetilde{\nabla f(\mathbf{x})})$, to quantify the variance of our estimator. Since $\boldsymbol{u}_i$ and $\boldsymbol{u}_j$ are independent random variables and have the same variance:.

\begin{equation}  \label{eqn:tv}
    \text{Var}(\widetilde{\nabla f(\mathbf{x})}) = \frac{1}{B} \text{Var}((\mathbf{u}_b\mathbf{u}_b^T)\nabla f(\mathbf{x}))
\end{equation}

\begin{align*} 
		\text{total variance} &= \text{tr}(\text{Var}(\widetilde{\nabla f(\mathbf{x})}) \\
		& = \text{tr}(\mathbb{E}[\widetilde{\nabla f(\mathbf{x})} \widetilde{\nabla f(\mathbf{x})} ^T]) - \text{tr}(\mathbb{E}[\widetilde{\nabla f(\mathbf{x})}]\mathbb{E}[\widetilde{\nabla f(\mathbf{x})}]^T)\\
		& = \frac{1}{B}(\nabla f(\mathbf{x})^T \mathbb{E}[\boldsymbol{u}_b \boldsymbol{u}_b^T \boldsymbol{u}_b \boldsymbol{u}_b^T] \nabla f(\mathbf{x}) - \\ 
		& \mathbb{E}[\widetilde{\nabla f(\mathbf{x})}]^T\mathbb{E}[\widetilde{\nabla f(\mathbf{x})}])
\end{align*}

Next, we will quantify the term $\mathbb{E}[\boldsymbol{u}_b \boldsymbol{u}_b^T \boldsymbol{u}_b \boldsymbol{u}_b^T]$. By Isserlis’ theorem, the odd order moment  $\mathbb{E}[\hat{u}_i \hat{u}_j \hat{u}_k]$ and $\mathbb{E}[\hat{u}_i]$ equal to 0:

\begin{align*}\label{eqnn:uuuu}
    \mathbb{E}[\boldsymbol{u}_b \boldsymbol{u}_b^T \boldsymbol{u}_b \boldsymbol{u}_b^T] &= \mathbb{E}[(\hat{\mathbf{u}} + \hat{\mathbf{e}})(\hat{\mathbf{u}} + \hat{\mathbf{e}})^T(\hat{\mathbf{u}} + \hat{\mathbf{e}})(\hat{\mathbf{u}} + \hat{\mathbf{e}})^T] \\
    &= \mathbb{E}[\hat{\mathbf{u}}\hat{\mathbf{u}}^T\hat{\mathbf{u}}\hat{\mathbf{u}}^T] + 2 \mathbb{E}[\hat{\mathbf{e}}\hat{\mathbf{e}}^T\hat{\mathbf{u}}\hat{\mathbf{u}}^T] +  \\
    & 4 \mathbb{E}[\hat{\mathbf{e}} \hat{\mathbf{u}}^T \hat{\mathbf{e}} \hat{\mathbf{u}}^T] + \mathbb{E}[\hat{\mathbf{e}}\hat{\mathbf{e}}^T\hat{\mathbf{e}}\hat{\mathbf{e}}^T]
\end{align*}

We can observe that $\mathbb{E}[\hat{\mathbf{e}} \hat{\mathbf{u}}^T \hat{\mathbf{e}} \hat{\mathbf{u}}^T] = \hat{G}\hat{\Sigma}$, which is by noticing that $\mathbb{E}[\hat{\mathbf{e}} \hat{\mathbf{u}}^T \hat{\mathbf{e}} \hat{\mathbf{u}}^T]_{i,j} = \hat{e}_i\hat{e}_j \mathbb{E}[\hat{u}_j^2]$. Similarly, we can also observe that $\mathbb{E}[\hat{\mathbf{e}}\hat{\mathbf{e}}^T\hat{\mathbf{u}}\hat{\mathbf{u}}^T]= \hat{G}\hat{\Sigma}$.

By applying the Isserlis’ theorem again, we can simplify $\mathbb{E}[\hat{\mathbf{u}}\hat{\mathbf{u}}^T\hat{\mathbf{u}}\hat{\mathbf{u}}^T] = \text{tr}(\hat{\Sigma})\hat{\Sigma}+2\hat{\Sigma}^2$. Therefore, \eqref{eqnn:uuuu} equals:

\begin{align}
    \mathbb{E}[\boldsymbol{u}_b \boldsymbol{u}_b^T \boldsymbol{u}_b \boldsymbol{u}_b^T] &= \text{tr}(\hat{\Sigma})\hat{\Sigma}+2\hat{\Sigma}^2 + 6\hat{G}\hat{\Sigma} + \hat{G}^2
\end{align}

Then \eqref{eqn:tv} equals (by \eqref{eqnn:uuuu} and \eqref{eqn:mean}):


\begin{align*}
		\text{total variance} &= \frac{1}{B} (\nabla f(\mathbf{x})^T \mathbb{E}[\boldsymbol{u}_b \boldsymbol{u}_b^T \boldsymbol{u}_b \boldsymbol{u}_b^T] \nabla f(\mathbf{x}) - \\
		& \mathbb{E}[\widetilde{\nabla f(\mathbf{x})}]^T\mathbb{E}[\widetilde{\nabla f(\mathbf{x})}]) \\
		&= \frac{1}{B}(\nabla f(\mathbf{x})^T \mathbb{E}[\boldsymbol{u}_b \boldsymbol{u}_b^T \boldsymbol{u}_b \boldsymbol{u}_b^T] \nabla f(\mathbf{x}) - \\ 
		& \nabla f(\mathbf{x})^T(\hat \Sigma+\hat G)(\hat \Sigma+\hat G)\nabla f(\mathbf{x})) \\ 
		& = \frac{1}{B}(\nabla f(\mathbf{x})^T (\text{tr}(\hat{\Sigma})\hat{\Sigma}+\hat{\Sigma}^2 + 4\hat{G}\hat{\Sigma}) \nabla f(\mathbf{x}))
\end{align*}


Since $\hat \Sigma=\lambda I$ and $\hat G = (1-\lambda)\boldsymbol{e} \boldsymbol{e}^T$, then the above equals:

\begin{align*}
    \text{total variance} &= \frac{1}{B}(\nabla f(\mathbf{x})^T (\lambda^2(n+1)I+ \\
    & 4(1-\lambda)\lambda \boldsymbol{e} \boldsymbol{e}^T ) \nabla f(\mathbf{x})) \\
    & = \frac{1}{B}(\lambda^2(n+1)||\nabla f(\mathbf{x})||_2^2 + \\
    & 4(1-\lambda)\lambda (\nabla f(\mathbf{x})^T \boldsymbol{e})^2)
\end{align*}

Especially,

\begin{equation*}
    \text{total variance} = \left\{\begin{array}{ll}
        \frac{n+1}{B}||\nabla f(\mathbf{x})||_2^2, & \text{when } \lambda=1\\
        % \lambda^2(n+1)||\nabla f(\mathbf{x})||_2^2 + 4(1-\lambda) (\nabla f(\mathbf{x})^T \boldsymbol{e})^2, & 0 \leq \lambda \leq 1\\
        0, & \lambda=0
        \end{array}
        \right.
\end{equation*}

$(n+1)||\nabla f(\mathbf{x})||_2^2 \gg 4 (\nabla f(\mathbf{x})^T \boldsymbol{e})^2 $ since $n$ is typically larger than 1 for high dimensional data such as images and $||\nabla f(\mathbf{x})||_2^2 \geq (\nabla f(\mathbf{x})^T \boldsymbol{e})^2$. Therefore, when $\lambda$ is close to 0, i.e., the search direction is more relying on the prior explanation, the variance will be much lower than the case where no search direction is provided.

\section*{EGSA: the optimal approximation}\label{sec:opt_approx}
Similarly, instead of changing the mean of the search distribution using the transfer prior, \cite{cheng2019improving} shape the covariance of the distrbution by $\mathbf{u}_b = \sqrt{\lambda} \mathbf{u} + \sqrt{1-\lambda}u' \mathbf{e}$ where $u'\sim\mathcal{N}(0,1)$ to trades off variance between the full parameter space and the prior space. In this way, changing $\mathbf{u}_b$ in the above manner is theoretically equivalent to adapting the covariance matrix of the sampling distribution \cite{cheng2019improving}:

\begin{equation}\label{eqn: sigma}
    \mathbf{\Sigma} = \lambda \epsilon \mathbf{I} + (1-\lambda) \mathbf{e}\mathbf{e}^T
\end{equation}

% In this attack, we consider a specific class of saliency maps that are generated using the absolute value of the gradient (ignoring their sign) such as in~\cite{simonyan2013deep, smilkov2017smoothgrad}. Thus, ${\bf e}_i = |E({\bf g}_i)|$. In this case, setting ${\bf e}$ as the transferrable prior and using the covariance matrix specified in Eqn.~\eqref{eqn: sigma} will lead to noisy estimation of the gradient as $\mathbb{E}[u_{b,i},u_{b,j}]={\bf e}_i {\bf e}_j= |E(\mathbf g_i)E(\mathbf g_j)| \neq E(\mathbf g_i)E(\mathbf g_j)$ for $i\neq j$. 
% %%% Pengrui what does this statement mean
% Note that at the diagonal of the covariance matrix $\mathbf{\Sigma}$, $\sigma_{i,i} = \lambda\epsilon + (1-\lambda)\mathbf{e_i}^2 = \lambda\epsilon + (1-\lambda)|\mathbf{e_i}|^2 = \lambda\epsilon + (1-\lambda)(E({\bf g}_i))^2$ if $\mathbf{e}$ is set as the transfer prior in Eqn. \eqref{eqn: sigma}. We therefore proposed EGSA by element-wise scaling:
In this attack, we proposed EGSA by element-wise scaling:

\begin{equation}\label{eq:transfer_sample}
    \mathbf{u}_b = \sqrt{\lambda} \mathbf{u} + \sqrt{1-\lambda} \mathbf{|e|} \odot \mathbf{u}
\end{equation} 

Therefore, the covariance matrix of the search distribution as follows:
\begin{equation}\label{eq:transfer}
    \mathbf{\Sigma^*} = \lambda \epsilon \mathbf{I} + (1-\lambda) \text{diag}(\mathbf{|e|}\odot\mathbf{|e|})
\end{equation}

The benefit of shaping the covariance matrix as $\mathbf{\Sigma^*}$ is that it provides us a substitution for $\mathbf{\Sigma}$ when the off-diagonal terms $\sigma_{i,j}$ are not available. In the followings, we show that $\mathbf{\Sigma^*}$ is the minimizer of the \textit{KL divergence} between the distribution $\mathcal N(\mathbf{0}, \mathbf{\Sigma})$ and the distribution $\mathcal N(\mathbf{0}, \mathbf{\Sigma'})$ for any $\mathbf{\Sigma'} \in \mathbb{D}=  \{\text{diag}(\sigma_{11},...\sigma_{NN}) | \sigma_{ii} \geq 0 \text{ for }\forall i \in [1,...,N]\}$. 

\begin{Proposition}
Denote $\mathcal{D}_1 = \mathcal N(\mathbf{0}, \mathbf{\Sigma})$ where $\mathbf{\Sigma}$ is shown in Eqn. \eqref{eqn: sigma}. For any Gaussian distribution $\mathcal{D}_2 \in \{\mathcal N(\mathbf{0}, \mathbf{\Sigma}')|\mathbf{\Sigma}'\in \mathbb{D}\}$, $\mathbf{\Sigma^*}$ minimizes the \textit{KL divergence} between $\mathcal{D}_1$ and $\mathcal{D}_2$.
\end{Proposition}
% \noindent \textbf{Proposition. 1} Denote $\mathcal{D}_1 = \mathcal N(\mathbf{0}, \mathbf{\Sigma})$ where $\mathbf{\Sigma}$ is shown in Eqn. \eqref{eqn: sigma}. For any Gaussian distribution $\mathcal{D}_2 \in \{\mathcal N(\mathbf{0}, \mathbf{\Sigma}')|\mathbf{\Sigma}'\in \mathbb{D}\}$, $\mathbf{\Sigma^*}$ minimizes the \textit{KL divergence} between $\mathcal{D}_1$ and $\mathcal{D}_2$.

\begin{proof}

% Let's denote $\mathcal{D}_1 = \mathcal N(\mathbf{0}, \mathbf{\Sigma})$ and  $\mathcal{D}_2 = \mathcal N(\mathbf{0}, \mathbf{\Sigma}')$. 
The \textit{KL divergence} is $D_{KL}(\mathcal{D}_1||\mathcal{D}_2)=\frac{1}{2}[\text{log}\frac{|\mathbf{\Sigma}_2|}{|\mathbf{\Sigma}_1|} - n +\text{tr}(\mathbf{\Sigma}_2^{-1}\mathbf{\Sigma}_1)+(\boldsymbol{\mu}_1-\boldsymbol{\mu}_2)^T\mathbf{\Sigma}_2^{-1}(\boldsymbol{\mu}_1-\boldsymbol{\mu}_2)]$. From assumption, we know that both $\mathcal{D}_1$ and $\mathcal{D}_2$ have zero mean. Then $D_{KL}(\mathcal{D}_1||\mathcal{D}_2)=\frac{1}{2}[\text{log}\frac{|\mathbf{\Sigma}_2|}{|\mathbf{\Sigma}_1|} - n +\text{tr}(\mathbf{\Sigma}_2^{-1}\mathbf{\Sigma}_1)]$.

% \begin{equation}\label{eqn: sigma}
%     \mathbf{\Sigma} = \lambda \epsilon \mathbf{I} + (1-\lambda) \mathbf{g}\mathbf{g}^T = \lambda \epsilon \mathbf{I} + (1-\lambda) (\mathbf{E}\odot\mathbf{q})(\mathbf{E}\odot\mathbf{q})^T
% \end{equation}

We can formulate the optimization problem as follows:

	\begin{subequations}\label{L2_loss}
		\begin{alignat}{2}
		&\underset{\mathbf\Sigma'}{\text{minimize}}& \qquad & D_{KL}(\mathcal{D}_1||\mathcal{D}_2)\\
		&\text{s.t.} & & \mathbf \Sigma' \in \mathbb{D} \\
		&& & \mathbf{\Sigma} = \lambda \epsilon \mathbf{I} + (1-\lambda) \mathbf{e}\mathbf{e}^T
		\end{alignat}
	\end{subequations}

% By eigenvalue decomposition, we denote $\mathbf{\Sigma} = \mathbf{U}\mathbf{\Lambda}_1 \mathbf{U}^T$, where $\mathbf{U} = [\mathbf{u}_1, ..., \mathbf{u}_n]$ and $\mathbf{u}_1 = \mathbf{\mathbf{E}\odot\mathbf{q}}$. Similarly,  $\mathbf{\Sigma}' = \mathbf{U}\mathbf{\Lambda}_2 \mathbf{U}^T$.

Further simplification leads to, $D_{KL}(\mathcal{D}_1||\mathcal{D}_2)=\frac{1}{2}[\sum_{i=1}^n\text{log}\sigma'_{ii}-\sum_{i=1}^n\text{log}\sigma_{ii}-n+\sum_{i=1}^n{\sigma'_{ii}}^{-1}\sigma_{ii}]$. Then the partial derivative with respect to each $\sigma'_{ii}$ is $\frac{\partial}{\partial \sigma'_{ii} }D_{KL}(\mathcal{D}_1||\mathcal{D}_2) ={\sigma'_{ii}}^{-1}-{\sigma'_{ii}}^{-2}\sigma_{ii}$. By setting the derivative to $0$, we can find the minimizer of each $\sigma'_{ii}=\sigma_{ii}$. This effectively tells us that the $\mathcal{D^*}=\mathcal{N}(\mathbf{0}, \mathbf{\Sigma^*})$ is a close approximation of the distribution $\mathcal{D}_1=\mathcal{N}(\mathbf{0}, \mathbf{\Sigma})$.
\end{proof}

The above discussion indicates that given the explanation $\mathbf E$, the attacker can incorporate it as the transfer prior through Eqn. \eqref{eq:transfer} since this will render a closer \textit{KL divergence} than any other distribution with a diagonal matrix. 

\section*{Dataset information}\label{sec:dataset}
\noindent \textbf{CIFAR-10. \cite{krizhevsky2009learning}} This is a benchmark dataset used to evaluate image recognition algorithms. The image is composed of 32×32 color images in 10 classes, with 6,000 images per class. 

\noindent \textbf{Purchases. \cite{shokri2017membership}} This is based on Kaggle’s “acquire valued shoppers” challenge dataset that contains shopping histories for several thousand consumers. Each individual record is a binary vector of 600 dimensions and there are 100 classes in total.

\noindent \textbf{Texas. \cite{shokri2017membership}} This dataset is based on the Hospital Discharge Data public use files with information about inpatients stays in several health facilities. Each individual record is a binary vector of 6170 dimensions and there are 100 classes in total.

\noindent \textbf{Human Activity Recognition (HAR). \cite{li2021units, roggen2010collecting}} This dataset in used for human locomotion recognition uses wearable motion sensors with inertial measurement units (IMU). Following \cite{li2021units}, each data example is a $45 \times 256$ matrix and there are 4 classes in total.

\noindent \textbf{Covid. \cite{rahman_2021}} This is a database of chest X-ray images to aid Covid-19 pneumonia diagnose, including 4 classes of COVID-19, normal, Viral Pneumonia, and Lung Opacity.

\section*{Acknowledgement}
The research presented in this paper is supported in part by the CONIX Research Center, one of
six centers in JUMP, a Semiconductor Research Corporation (SRC) program sponsored by DARPA,
the U.S. Army Research Laboratory and the U.K. Ministry of Defence under Agreement Number
W911NF-16-3-0001 and the National Science Foundation (NSF) under award \# CNS-1822935, and
by the National Institutes of Health (NIH) award \# P41EB028242 for the mDOT Center. The views
and conclusions contained in this document are those of the authors and should not be interpreted as
representing the official policies, either expressed or implied, of the NSF, the NIH, the U.S. Army
Research Laboratory, the U.S. Government, the U.K. Ministry of Defence or the U.K. Government.
The U.S. and U.K. Governments are authorized to reproduce and distribute reprints for Government
purposes notwithstanding any copyright notation hereon. This work has been submitted to the IEEE for possible publication. Copyright may be transferred without notice, after which this version may no longer be accessible.
%We therefore name this strategy as Explanation-guided Sampling Attack (EGSA).\\

% \section{Combine with low-dimensional transfer prior}\label{qeba}

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/atk_success-qeba-h.eps} \centering  \par
%     \endminipage\hfill
%     \vspace{-0.5em}
% 		\caption{Attack success rate of hard-label attack combining with low-dimensional transfer prior}
% 	\label{fig:MEA-covid}
% % 	\vspace{-.5em}
% \end{figure}


% \section{DP-based provable defense}
% \label{sec:defense}

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/DP_softlabel_gradient/f_val-17.eps} 
%         % \centering (a) Grad (true):Loss\par
%     \endminipage\hfill
%     \caption{Grad (true):Loss for soft-label attack with true \textit{Gradient} explanation and DP-\textit{Gradient} explanation. The number denotes the DP scale parameter $b$}\label{fig:defense_soft_label_gradient_org}
% \end{figure}

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/DP_hardlabel_gradient/L2-abs.eps} 
%         % \centering (a) Grad (abs): L2-distance\par
%     \endminipage\hfill
%     \caption{(a) Grad (abs): L2-distance for hard-label attack with absolute-valued \textit{Gradient} explanation and DP-\textit{Gradient} explanation. The number denotes the DP scale parameter $b$}\label{fig:defense_hard_label_gradient_abs}
% \end{figure}

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/DP_hardlabel_gradient/diff_cosine-17.eps} \centering (a) Grad: cosine similarity\par
%     \endminipage\hfill
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/DP_hardlabel_gradient/L2-27.eps} \centering (b) Grad (true): L2-distance \par
%     \endminipage\hfill
%     \caption{L2 for for hard-label attack with true \textit{Gradient} explanation and DP-\textit{Gradient} explanation. The number denotes the DP scale parameter $b$}\label{fig:defense_hard_label_gradient_org}
% \end{figure}

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/DP_hardlabel_ig/diff_cosine-20.eps} \centering (a) IntegratedGradients: cosine similarity\par
%     \endminipage\hfill
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/DP_hardlabel_ig/L2-36.eps} \centering (b) IntegratedGradients (true): L2-distance \par
%     \endminipage\hfill
%     \caption{L2 for hard-label attack with true \textit{IntegratedGradients} explanation and DP-\textit{IntegratedGradients} explanation. The number denotes the DP scale parameter $b$}\label{fig:defense_hard_label_ig_org}
% \end{figure}

% In this section, we describe the mechanism that we employ to generate differential private (DP) explanations. We adopt the ideas in~\cite{abadi2016deep} to generate DP explanations. An overview of the explanation generation pipeline is provided in Fig.~\ref{fig:flow_dp}. 
% % Using DP-SGD to train models~\cite{abadi2016deep}, or use of a DP-based noise layer to provide certifiable robustness~\cite{lecuyer2019certified} has been proposed in prior work. In this paper, we adopt the ideas to generate DP-explanation. 
% \begin{figure}[h]
% \includegraphics[width=0.9\linewidth]{images/defense_pipeline.png}  \centering
% 	\caption{Differential Private Explanation Pipeline.}
% 	\end{figure}\label{fig:flow_dp}
% The differentially private mechanism is denoted by $\mathcal{K}$ and the gradient-based explanation mechanism is denoted by $E$.
% % The DP-mechanism $\mathcal{K}$, takes an input $\mathbf g$ and performs the following two-step process below:
% % \begin{itemize}[leftmargin=*]
% %     \item {\bf Step 1: Gradient Clipping:} We set a clipping threshold $C$ and clip the gradient vector as $\hat{\mathbf g} = \frac{\mathbf g}{\max(1, \frac{||\mathbf g||_2}{C}) }$.
% %     \item {\bf Step 2: Add Laplace Noise:} Add noise vector $\eta \in \mathbb{R}^N$ to $\hat{\mathbf g}$. The noise vector $\eta$ is sampled from a Laplace distribution $Lap(0, b)$ with scale $b=\frac{C}{\epsilon}$ where $\epsilon$ is a user chosen privacy parameter. Each dimension of $\eta$ is independently sampled.
% % \end{itemize}

% % \begin{Proposition}
% % The mechanism $\mathcal{K}$ described above preserves $\epsilon-$differential privacy. Formally, for any two gradient vectors $\mathbf g$ and $\mathbf g'$ and some $s \in \mathbb{R}^N$ we have:
% % \[ Pr(\mathcal{K}(\mathbf g) = s) \leq e^{\epsilon} Pr(\mathcal{K}(\mathbf g') = s) \]
% % \end{Proposition}

% % \begin{proof}
% % By construction, steps 1 and 2 when applied together satisfy $\epsilon-$differential privacy~\cite{abadi2016deep, dp_book}.
% % \end{proof}

% % We now show that the explanation generation module, which is a composition of $\mathcal{K}$ and the explanation mechanism $\mathbf E$ is also $\epsilon-$differentially private. 

% % \begin{Proposition}
% % Formally, for any two gradient vectors $\mathbf g$ and $\mathbf g'$ and some $s \in \mathbb{R}^N$ we have:
% % \[ Pr({\mathbf E}(\mathcal{K}(\mathbf g)) = s) \leq e^{\epsilon} Pr({\mathbf E}(\mathcal{K}(\mathbf g')) = s) \]
% % \end{Proposition}

% % \begin{proof}
% % Using post-processing invariance property of differential privacy~\cite{dp_book}.
% % \end{proof}

% For ease of exposition, we denote the gradient vector ${\bf g} = \nabla_{\bf x} F({\bf x})_i$ for some label $i \in [k]$. 
% The idea is to intercept the gradient vector of the model, and make it differentially private (DP) before it is shared with the explanation mechanism $E$. 
% As shown in Fig.~\ref{fig:flow_dp} we define the DP-mechanism $\mathcal{K}$ as a two-step process as follows:
% \begin{enumerate}
% \item {\bf Gradient Clipping}: We set a clipping threshold $C \in \mathbb{R}$ and clip the gradient vector as:
% \[ {\bf \hat{g}} = \frac{{\bf g}}{\max({1, \frac{||{\bf g}||_2}{C}})} \]
% %\[ {\bf \hat{g}} = \frac{{\bf g}}{\max({1, \frac{||{\bf g}||_1}{C}})} \]
% This bounds the sensitivity of the gradient vector by ensuring that $|| {\bf g} ||_2 \leq C$.
% %This bounds the sensitivity of the gradient vector by ensuring that $|| {\bf g} ||_1 \leq C$.

% \item {\bf Add Laplace Noise}: We draw noise vector $\eta \in \mathbb{R}^{n}$ from a Laplace distribution $Lap(0, b)$ 
% where $b = \frac{C}{\frac{\epsilon} {2\sqrt{n}}}$. 
% %where $b = \frac{C}{\epsilon}$.
% The parameter $\epsilon$ is user specified and denotes the privacy level. A lower value of $\epsilon$ implies higher privacy. Each dimension of the vector, $\eta_{i}$ for $i = 1, \ldots, n$ is sampled independently from the distribution. The noise vector is added to the clipped gradient to generate $\bf{\tilde{g}}$ as:
% \[ {\bf \tilde{g}} = {\bf \hat{g}} +  \eta \]
% \end{enumerate}

% \begin{Proposition}
% The two-step DP-mechanism $\mathcal{K}$ described above is $\epsilon-$differentially private. Formally, for any two gradient vectors ${\bf g}$ and ${\bf g'}$ and some ${\bf s} \in \mathbb{R}^m$ we have:
% \[ Pr(\mathcal{K}({\bf g}) = {\bf s}) \leq e^{\epsilon} Pr(\mathcal{K}({\bf g'}) = {\bf s}) \]
% \end{Proposition}

% \begin{proof}
% \begin{eqnarray}
% \frac{Pr(\mathcal{K}({\bf g}) = s)}{Pr(\mathcal{K}({\bf g'}) = s)} &=& \prod_{i=1}^{m} \frac{\exp(-| {\bf g}_i - \bf{s}_i |/b)}{\exp(-| {\bf g'}_i - \bf{s}_i |/b)} \label{eqn:laplace} \\
% & \leq & \prod_{i=1}^{m} \exp( | {\bf g'}_i - {\bf g}_i | / b) \label{eqn:inequality} \\
% \log \frac{Pr(\mathcal{K}({\bf g}) = s)}{Pr(\mathcal{K}({\bf g'}) = s)} & = & \sum_{i = 1}^m | {\bf g'}_i - {\bf g}_i | / b \label{eqn:log} \\
% & \leq & \sqrt{n} || {\bf g'} - {\bf g} ||_2 / b \label{eqn:l2norm} \\
% %& = & || {\bf g'} - {\bf g} ||_1 / b \label{eqn:l1norm} \\
% & \leq & 2 \sqrt{n} C / b \label{eqn:triangle} \\
% & = & \epsilon \nonumber
% \end{eqnarray}
% \end{proof} 
% Eqn.~\eqref{eqn:laplace} is due to the noise vector drawn from the Laplace distribution, Eqn.\eqref{eqn:inequality} is obtained by applying triangle inequality. Taking logarithm on both sides in Eqn.~\eqref{eqn:log} and using the definition of $l_2$-norm we get Eqn.~\eqref{eqn:l2norm}. Replacing the value of $b$ completes the proof. 

% The explanation mechanism $E$, takes as input the DP gradient vector $\mathcal{K}({\bf g})$ and provides as explanation ${\bf e} \in \mathbb{R}^n$. We now show that the explanation mechanism $E$ is also differentially private. 

% \begin{Proposition}
% For any two gradient vectors, ${\bf g}$ and ${\bf g'}$, and some explanation ${\bf e}$, the gradient-based explanation mechanism $E$ is $\epsilon-$differentially private. Formally, 
% \[ Pr(E[\mathcal{K}({\bf g})] = {\bf e}) \leq e^{\epsilon} Pr(E[\mathcal{K}({\bf g'})] = {\bf e}) \]
% \end{Proposition}
% \begin{proof}
% Using post-processing invariance property of differential privacy~\cite{dp_book}.
% \end{proof}



% \subsection{Results Using Differentially Private Explanations}
% \noindent{\textbf{Defending the explanation.}} This section presents the evaluation results of our Differential Privacy(DP)-based provable defense, using Gradient and Integrated Gradient explanations. We do this because based on our attacks, and quite understandably so, we found Gradient explanation to leak the maximum information about the gradient vector. We generate DP-explanations by varying the scale parameter $b=\frac{C}{\epsilon}$ of the Laplace distribution. We keep $C=1$ and vary the value of the privacy parameter $b=\frac{1}{\epsilon} = 0.001, 0.01, 0.1 \text{ and etc.}$. Thus, the higher the scale parameter $b$, the stronger the privacy. We then use these DP explanations for performing both soft- and hard-label attacks and report results. 

% Fig. \ref{fig:defense_soft_label_gradient_org} shows the expected loss $\mathbb{E}[\mathcal{L}(\mathbf{x})]$ versus the number of queries consumed in the soft-label attack when using DP-explanations. We can see that using DP-explanations can effectively make the soft-label attack converge slower than using the explanation directly obtained from the explanation methods. Using a DP-scale of 0.1 is sufficient to protect the attack. Similarly, Fig. \ref{fig:defense_hard_label_gradient_abs}, \ref{fig:defense_hard_label_gradient_org}, and \ref{fig:defense_hard_label_ig_org} plots the mean $L_2$ distance between $\mathbf{x}$ and the adversarial example on the y-axis versus the number of queries in x-axis in the hard-label setting. We again see that the defended true explanation can make the attack as inefficient as the baseline approach. Besides, we can also observe that from the defender perspective, a good value for DP-scale is above 0.01 as this significantly reduces the leakage of gradient information. A noise magnitude less than this is insufficient to provide protection. At the same time, the DP-noise level shouldn't be too large as that will compromise the utility of explanations. Overall, this demonstrates that the DP-explanations can effectively make the gradient estimation harder and reduce the attackers' advantage. 


% \noindent{\textbf{Bypass the Defense using running averages.}} In Fig. \ref{fig:bypass_defense_hard_label_gradient_org} and \ref{fig:bypass_defense_hard_label_ig_org} we show one approach to bypass the defense using the running average of explanations at a specific iteration. We denote the number as scale $b$ used in Laplace distribution and the number after underscore as the number of samples to estimate the mean. For EGTA approach, when the explanation is incorporated into the attack algorithm by Eqn.\eqref{eq:direct_transfer}, the attack will request multiple inferences and use the mean of explanations to replace the current returned explanation. Fig. \ref{fig:bypass_defense_hard_label_gradient_org} (a) shows that using the mean of explanations can effectively increase the cosine similarity, even using mean of two can increase the cosine similairy by at least 1 time. Second, in Fig. \ref{fig:bypass_defense_hard_label_gradient_org} (b), we can observe that using the mean of 2 explanations or equivalently increase the cosine similarity above 0.2 can already effectively bypass the DP-defense. In Fig. \ref{fig:bypass_defense_hard_label_gradient_org} we also observe a similar trend but the risk of mean is less serve. For instance, in Fig. \ref{fig:bypass_defense_hard_label_gradient_org} (b), while an average of 50 samples is sufficient to defeat the DP-defense, only 2 of samples will work in the case of \textit{Gradient} explanation in Fig. \ref{fig:bypass_defense_hard_label_gradient_org} (a). We believe this is due to the non-linearity of the \textit{IntegratedGradients} as a function of \textit{Gradient}. This will affect the efficacy of using average to estimate the expectation of random variables. And we expect a similar behavior will also exist for other explanations which have a complex transformation of the \textit{Gradient} explanation.

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/DP_hardlabel_gradient_bypass/diff_cosine-19.eps} \centering (a) Cosine similarity\par
%     \endminipage\hfill
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/DP_hardlabel_gradient_bypass/L2-35.eps} \centering (b) L2-distance \par
%     \endminipage\hfill
%     \caption{Bypass the DP-defense for hard-label attack with DP-\textit{Gradient} explanation. The first number denotes the DP scale parameter $b$ and the second number denotes the number of explanation samples used to estimate the mean}\label{fig:bypass_defense_hard_label_gradient_org}
% \end{figure}

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/DP_hardlabel_ig_bypass/diff_cosine-18.eps} \centering (a) Bypass defense IntegratedGradients: cosine similarity\par
%     \endminipage\hfill
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/DP_hardlabel_ig_bypass/L2-34.eps} \centering (b) Bypass defense IntegratedGradients: L2-distance \par
%     \endminipage\hfill
%     \caption{Bypass the DP-defense for hard-label attack with DP-\textit{IntegratedGradients} explanation. The first number denotes the DP scale parameter $b$ and the second number denotes the number of explanation samples used to estimate the mean}\label{fig:bypass_defense_hard_label_ig_org}
% \end{figure}
	

% \noindent{\textbf{Maintaining explanation utility.}} 
% %While defending against the attack using explanation, one should also maintain the utility of the explanation. 
% %By building the DP-provable defense, we trade the faithfulness to the true explanation against the privacy of the gradient direction. 
% Differentially private explanations are generated by adding designed noise. Therefore, it is useful to quantify the \emph{utility} of a DP-explanation. A good DP-explanation must satisfy the following two properties. 1) Should highlight relatively the same portion of the image as the original explanation so that it looks visually similar. 2)The explanations should be clear enough that a user can classify the original image based on the explanation.  

% To measure the first property, we adopt the quality estimation metric PSNR that evaluates the distance between the DP-explanation and the original, undefended explanation. And to evaluate the second property, we will use the true explanations and DP explanations to mask the original images and then partition those masked images into a training and test set. We then train a neural network to classify the masked images and measure its performance. In this method, the neural network model acts as a proxy for the user to classify the images. If the neural network can classify with a good accuracy and if the DP-explanation has a high PSNR, then the utility of the explanation in preserved. 

% From Fig. \ref{fig:utility-cifar10}, we perform such evaluation on CIFAR10 and can observe that the mean $L_2$ distance increases using 5000 queries of the victim models as we have stronger privacy. Besides, the PSNR values decrease but saturate at around 20 \textit{dB}. Since an acceptable PSNR range from image compression is about 20 \textit{dB} to 25 \textit{dB} \cite{huynh2012accuracy, huynh2008scope}, we conclude the utility of explanations are mainly preserved. Besides, we can also observe that the model trained on these masked image datasets also maintains accuracy when the DP scale level $b$ is 0.01 or less. We think this is a reasonable range to trade-off for stronger privacy. 

% From Fig. \ref{fig:utility-imagenet}, we can also observe a similar trend on ImageNet dataset. The attack efficacy decrease (as the $L_2$ distance increases) when the explanation has stronger privacy. On the other hand, the PSNR values decrease and get saturated. Hence we think choosing the DP scale $b=0.01$ is reasonable to maintain utility and defend against explanation-guided attacks.

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/utility/cifar10_test-2.eps} 
%         % \centering (a) Grad (true):Loss\par
%     \endminipage\hfill
%     \caption{The utility of different DP-\textit{IntegratedGradients} on CIFAR10 test dataset. x-axis is the DP-scale $b$. Higher the value, stronger the privacy. $L_2$ is the mean $L_2$ distance for hard-label attack using DP explanations with different scale $b$ and query budget 5000. PSNR denotes the PSNR value between the true explanation and the DP-generated explanation. Accuracy denotes the model trained on DP-explanations-masking images. The plot shows that as the scale $b$ increases, the PSNR decreases but quickly get saturated and the performance of the model degrades.}\label{fig:utility-cifar10}
% \end{figure}

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/utility/imagenet_test.eps} 
%         % \centering (a) Grad (true):Loss\par
%     \endminipage\hfill
%     \caption{The utility of different DP-\textit{IntegratedGradients} on ImageNet test dataset. x-axis is the DP-scale $b$. Higher the value, stronger the privacy. $L_2$ is the mean $L_2$ distance for hard-label attack using DP explanations with different scale $b$ and query budget 5000. PSNR denotes the PSNR value between the true explanation and the DP-generated explanation.}\label{fig:utility-imagenet}
% \end{figure}

% Fig.~\ref{fig:vis} shows the original explanation and the DP-explanations generated using Gradient and Integrated Gradients. 
% %DP-explanations changes the scale parameter of the Laplace distribution which controls the level of privacy. 
% The pixel of the top-10\% highest values are selected and are then  multiplied by the original image to extract the semantic information. As shown in Fig. \ref{fig:vis}, DP-explanations using both Gradient and Integrated Gradients highlight the location of the \emph{gazelle} in the image indicating that they continue to preserve the semantic integrity of the original explanation. This visually verifies that our defense approach can maintain the fidelity of the explanation while reducing the attack efficiency as shown by the previous experiments. Besides, we also plot the Peak signal-to-noise ratio (PSNR) values between the true explanation and the DP-generated explanation. For instance, the DP-\textit{Gradient} explanations typically have PSNR from 19.61dB to 31.45dB. Since acceptable PSNRs are considered to be above 20 dB based on wireless image compression, we can conclude that the DP-explanation is still acceptable.

% 	\begin{figure*}[h]
%     \minipage{0.18\textwidth}
%         \includegraphics[width=\linewidth]{images/vis_1/original-5.jpg} \centering original image\par
%     \endminipage\hfill
%     \minipage{0.18\textwidth}
%         \includegraphics[width=\linewidth]{images/vis_grad/Gradient_0_top_org_cls_354_ssim_0.7351.png} \centering Grad \par
%     \endminipage\hfill
%     \minipage{0.18\textwidth}
%         \includegraphics[width=\linewidth]{images/vis_grad/Gradient_0_top_sur_cls_354_ssim_0.7351.png} \centering  Grad-0.001 (31.45dB) \par
%     \endminipage\hfill
%     \minipage{0.18\textwidth}
%         \includegraphics[width=\linewidth]{images/vis_grad/Gradient_0.01.png} \centering  Grad-0.01 (19.81dB) \par
%     \endminipage\hfill
%     \minipage{0.18\textwidth}
%         \includegraphics[width=\linewidth]{images/vis_grad/Gradient_0.1.png} \centering  Grad-0.1 (19.61dB) \par
%     \endminipage\hfill
%     \\
%     \minipage{0.18\textwidth}
%         \includegraphics[width=\linewidth]{images/vis_1/original-5.jpg} \centering original image\par
%     \endminipage\hfill
%     \minipage{0.18\textwidth}
%         \includegraphics[width=\linewidth]{images/vis_ig/IntegratedGradients_0_top_org_cls_354_ssim_0.3777-1.png} \centering IG \par
%     \endminipage\hfill
%     \minipage{0.18\textwidth}
%         \includegraphics[width=\linewidth]{images/vis_ig/IntegratedGradients_0_top_sur_cls_354_ssim_0.3777-1.png} \centering IG-0.001 (25.09dB) \par
%     \endminipage\hfill
%     \minipage{0.18\textwidth}
%         \includegraphics[width=\linewidth]{images/vis_ig/IntegratedGradients_0.01.png} \centering  IG-0.01 (16.75dB) \par
%     \endminipage\hfill
%     \minipage{0.18\textwidth}
%         \includegraphics[width=\linewidth]{images/vis_ig/IntegratedGradients_0.1.png} \centering IG-0.1 (16.53dB) \par
%     \endminipage\hfill

%     \vspace{-0.5em}
% 		\caption{Visualization of different DP explanations. The first column is the explanation generated using Gradient information and the second column is Intergated Gradients (IG). From left to right, they are the original image, undefended explanation, DP explanations with different level of privacy with scale parameter equal to 0.001, 0.01, 0.1. We can visually verify that the DP provable defense preserve the utility by highlighting similar region whether the object locates.}
% 	\label{fig:vis}
% % 	\vspace{-.5em}
% 	\end{figure*}


==> TIFS-2022 (Arxiv) 2/discussion.tex <==
% \section{Discussion}
% \noindent{\textbf{Summary and key takeaways.}} We proposed and revisited several attacks that will compromise the security and privacy of machine learning models:
% \begin{itemize}
%     \item EA: The true gradient-based explanations, e.g., Gradient, Smooth Grad, and Integrated Gradients, can leak significant amount of information where the query budget is reduced by 10 times for soft-label and hard-label evasion attacks. The absolute-value explanation is less information-leaky but can still be used by the attacker to improve the efficiency by 2 times. Besides, for explanations with low cosine similarity to the true gradients, we further proposed the surrogate model-based attack and observed 5 times reduction compared to the baseline. It also produces better performance compared to existing transfer-based attacks.
%     \item MIA: Instead of claiming by the previous works that the advantages are limited for common explanations, such as Smooth Grad and LIME, we observe leakage of a significant amount of information about individual membership for various explanations consistently (by more than 100\% improvement). 
%     \item MEA: We observed that the advantage is modest compared to the baseline where no explanation is provided. For CIFAR10 annd MNIST dataset we observed 5 - 10 times improvement but limited improvement on Covid and HAR datasets. We empirically analyze the underlining reasons and found the MSV as a strong indicator of the MEA performance.
% \end{itemize}

% For each explanations, we also provide a summary of the information leaked based on the improvement on the attack efficiency in Table \ref{table:category}. We give high level of information leakage if the explanation can help improve the attack efficiency by 5 - 10 times; a medium level if the efficiency is increased by 2 - 5 times; and a low level if there is less than 2 times or barely no improvements.

% \begin{table}[]
% \small
% \begin{adjustbox}{max width=0.45\textwidth}
%     \begin{tabular}{c|c|c|c}
%     \hline
%     Explanation & EA & MIA & MEA \\ 
%     \hline
%     Gradient~\cite{simonyan2013deep} & high & high & medium \\
%     \hline
%     Guided-backprop~\cite{springenberg2014striving} & medium & high & medium \\
%     \hline
%     Smooth Grad~\cite{smilkov2017smoothgrad} & high & high & medium \\
%     \hline
%     Int. Grad~\cite{sundararajan2017axiomatic} & high & high & medium \\
%     \hline
%     Grad-Cam~\cite{selvaraju2017grad} & medium & high & medium \\
%     \hline
%     LIME~\cite{ribeiro2016should} & low & high & low \\
%     \hline
%     \end{tabular}
% \end{adjustbox}
% \caption{Risk categorization based on the level of information leakage from explanations and corresponding attacks.}\label{table:category}
% \vspace{-2em}
% \end{table}

\section{Discussion}
Our empirical analysis highlight that gradient-based explanations such as Gradient, SmoothGrad, and IntegratedGrad, allow an adversary to better estimate gradients in black-box settings. Therefore, attacks can be executed with lower number of queries (around $10\times$ for hard and soft label EA) making them efficient and increasing their feasibility in practice. Even when explanations reveal a function of the gradients (e.g., absolute value of gradients, LIME), our proposed attacks show improvement in attack efficiency ($2-5\times$ for EA, and increased leakage of membership information). However, for MEA the gains observed are modest ($5-10\times$ for CIFAR-10 and MNIST, and lower for Covid and HAR). We categorize the risk of explanation release into three classes based on the increase they cause in attack efficiency: high ($5-10\times$), medium ($2-5\times$) and low ($\leq 2\times$). We hope this will help practitioners in understanding the risks associated with explanation release and allow them to make informed decisions about the explanation technique to use.

There are other attacks that can be included as part of the risk profile. While we focused on attacks at model deployment time, there could be additional risks associated with training time attacks~\cite{shap_poisoning} as well. We emphasize that the goal of our study was not to be exhaustive but to initiate a systematic exploration of the interaction between explanations and privacy and security attacks and understand how different types of explanations effect risk. While our results indicate that explanations do represent an information-rich side-channel that can be exploited for improving attack efficiency, there is still work that needs to be done to make these attacks practical, especially in the access-constrained black-box settings.

==> TIFS-2022 (Arxiv) 2/experiments.tex <==
\section{Experiments}\label{sec:exps}
\subsection{Evasion attack (EA)}
We use the number of queries needed to achieve a particular attack success rate as the metric to measure attack efficiency across all experiments for both soft and hard-label attacks. The baseline attack is when the adversary has access to only the model output and no explanation. All our experiments have been performed on a ResNet-50~\cite{he2016deep} as the target model trained on ImageNet~\cite{deng2009imagenet} dataset. The reported values are obtained by averaging over successful attacks on $100$ correctly classified images. For the $\lambda$ used in \eqref{eq:direct_transfer}, we fix its value as 0.9 in the remaining experiments. 

In summary, we consider the true explanation and the absolute-value explanations returned to the attacker. The attacker will use the three proposed explanation-guided attack approaches. We omit the absolute-value explanations for EGTA and EGSMA due to inaccurate transfer information. We also exclude the true explanation for EGSA because it has the same performance as the absolute-value explanation. For EGSMA, We omit the results for LIME since the loss of $\mathcal{L}_{expln}$ is not differentiable over the surrogate model parameters and hence EGSMA cannot be directly applied.


% 	\begin{figure}[h]
%     \minipage{0.22\textwidth}
%         \includegraphics[width=\linewidth]{images/results/s-egta.eps} \centering (a) Soft-label\par
%     \endminipage\hfill
%     \minipage{0.22\textwidth}
%         \includegraphics[width=\linewidth]{images/results/h-egta.eps} \centering (b) hard-label\par
%     \endminipage\hfill

%     \vspace{-0.5em}
% 		\caption{Attack success rate of EGTA using the true explanations.Gradient, Int. Gradients, Guided BP and etc. stands for different explanations used in aiding the attacker. None stands for no additional information is used.}
% 	\label{fig:exps-soft-org}
% % 	\vspace{-.5em}
% 	\end{figure}

\begin{figure*}[t]
    \centering
    % \subfigure{
    \begin{minipage}{0.3\linewidth}
     \centering

    \includegraphics[width=\linewidth]{images/results/s-egta.png} \centering (a) Soft-label\par
    \includegraphics[width=\linewidth]{images/results/h-egta.eps} \centering (b) hard-label\par
    
    \caption{Attack success rate of EGTA using the true explanations.}
    \label{fig:exps-soft-org}
  \end{minipage}
%   }
    % \subfigure{
    \begin{minipage}{0.3\linewidth}
     \centering
    %  \vspace{-1.7cm}
  \includegraphics[width=\linewidth]{images/results/s-egsa.eps} \centering (a) Soft-label \par
  \includegraphics[width=\linewidth]{images/results/h-egsa.eps} \centering (b) Hard-label\par
    \caption{Attack success rate of EGSA using explanations with absolute values.}
    \label{fig:exps-soft-abs}
  \end{minipage}
%   }
%   \subfigure{
    \begin{minipage}{0.3\linewidth}
     \centering
    %  \vspace{-1.7cm}
     \includegraphics[width=\linewidth]{images/results/s-egsma.eps} \centering (a) Soft-label \par
     \includegraphics[width=\linewidth]{images/results/h-egsma.eps} \centering (b) Hard-label\par
    \caption{Attack success rate of EGSMA using true explanations.}
    \label{fig:exps-learn-s}
  \end{minipage}
%   }
%   \vspace{-20pt}
\end{figure*}

\subsubsection{Explanation-guided Transfer Attack (EGTA)}

\noindent \textbf{Soft-label attack results using true explanations:} We start with an image in the target class $t$ and try to generate perturbation such that it is misclassified to any other class by the model. We set $L_2=1.25$ as our perturbation budget to compare with \cite{cheng2019improving}. In Fig. \ref{fig:exps-soft-org} (a), we show the median attack success rate of achieving the target distortion with various queries consumed. First, we can see that our proposed approach of using the information from the Gradient, Integrated Gradient, and SmoothGrad can reduce the query budget by more than $\times 10$, indicating that gradient information is leaked by the above explanations. Besides, since this is an biased estimator, using Integrated Gradient and SmoothGrad explanations leads to suboptimal convergence. Hence, the attack success rate quickly saturates due to the bias in gradient estimation. Also, for explanations drastically different from Gradient, such as Guided Backprop and GradCam, the direct transfer attack (EGTA) may lead to poor attack performance due to biased gradient estimation.

% 	\begin{figure}[h]
%     \minipage{0.22\textwidth}
%         \includegraphics[width=\linewidth]{images/results/s-egsa.eps} \centering (a) Soft-label \par
%     \endminipage\hfill
%     \minipage{0.22\textwidth}
%         \includegraphics[width=\linewidth]{images/results/h-egsa.eps} \centering (b) Hard-label\par
%     \endminipage\hfill
% 		\caption{Attack success rate of EGSA using explanations with absolute values.}
% 	\label{fig:exps-soft-abs}
% 	\vspace{-1em}
% 	\end{figure}

%  	\begin{figure}[h]
%     \minipage{0.22\textwidth}
%         \includegraphics[width=\linewidth]{images/results/s-egsma.eps} \centering (a) Soft-label \par
%     \endminipage\hfill
%     \minipage{0.22\textwidth}
%         \includegraphics[width=\linewidth]{images/results/h-egsma.eps} \centering (b) Hard-label\par
%     \endminipage\hfill
% 		\caption{Attack success rate of EGSMA using true explanations.}
% 	\label{fig:exps-learn-s}
% 	\vspace{-1em}
% 	\end{figure}

\noindent \textbf{Hard-label attack results using true explanations:} In this setting, we consider a targeted attack. An attacker starts with an image in the target class and iteratively reduces the $L_2$ distance to the original image $\mathbf{x}$ to generate the adversarial image. Here we use the distortion threshold $L_2=12.5$ as the attack success metric because we empirically found that the noise magnitude is imperceptible. Fig. \ref{fig:exps-soft-org} (b) shows that having access to the explanation reduces the number of queries needed to reach the same attack success rate. For Gradient, IntegratedGradients, and Smooth Grad, the transfer attack can reduce the query budget by about 10 times. However, for other variants such as Guided Backprop and GradCam, directly using transfer attack leads to worse attack performance.

% \noindent \textbf{EGTA results using absolute-valued explanations:} In this case, EGTA leads to poor performance and we omit EGTA using absolute-valued explanations due to space limits. This issue can be further handled by our proposed approaches EGSA which will be discussed in the following sections.

\subsubsection{Explanation-Guided Sampling Attack  (EGSA)}
\noindent \textbf{Soft-label attack results using absolute-valued explanation:} The previous EGTA is only applicable to true explanations, but does not generalize to explanations with absolute values for visualization. Here we demonstrate that EGSA applies to the absolute-value explanations in Fig. \ref{fig:exps-soft-abs} (a). We can observe that the attack efficiency is significantly improved for Gradient, Smooth Grad, and Integrated Gradients by 3 -5 times. The improvement is limited for LIME, Guided Backprop, and GradCam. 

\noindent \textbf{Hard-label attack results using absolute-valued explanation:} Fig. \ref{fig:exps-soft-abs} (b) shows the attack efficiency by leveraging absolute-valued explanations. Similarly, we can observe that the attack efficiency is significantly improved for Gradient, Smooth Grad, and Integrated Gradients by 2 times. The improvement is limited for LIME, Guided Backprop, and GradCam. 

% Here we need to point out that EGSA will have the identical performance for the true explanations and the absolute-value explanations. Given the limitation of EGTA and EGSA where it does not works well for gradient variants that are more distinct from the true Gradient explanation, we further show that EGSMA can mitigate the drawbacks.

\subsubsection{Explanation-Guided  Surrogate  Model  Attack  (EGSMA)} 
\noindent \textbf{Soft-label attack results using true explanations:} In Fig \ref{fig:exps-learn-s} (a), we show the performance of EGSMA using various explanations. First, we can observe that EGSMA can robustly increase the attack performance by 10 times for Smooth Grad, and by 2-3 times for Integrated Gradients, GradCam, and Guided Backprop. Here, EGSMA can increase the performance of attacks when the direct transfer fails. Fig. \ref{fig:exps-learn-s} (a) also shows that EGSMA is a robust method where the attacks success rate increase consistently compared to EGTA where the direct transfer fails.

\noindent \textbf{Hard-label attack results using true explanations:} Fig \ref{fig:exps-learn-s} (b) shows the performance of EGSMA in hard-label setting. It produces 2 - 3 times improvment for SmoothGrad and IntegratedGradients.

% \noindent{\textbf{EGSMA results using absolute-valued explanations:}} Here when applying EGSMA to absolute-valued explanations, we observe that the quality of the gradient of the surrogate model does not increase, and using this surrogate gradient does not improve our performance. The reason is that due to the lost of the sign information of explanations, finetuning the surrogate model learns confusing gradient information.

\subsubsection{Attack results summary}

\begin{table*}[h]
	\centering
	\begin{adjustbox}{max width=0.85\textwidth}
		\begin{tabular}{c|c|cccc|cccc|cccc}
			\toprule
			% \multicolumn{2}{c}{Part}                   \\
			Atk. rate  & {None} & \multicolumn{4}{c}{Smooth Grad } & \multicolumn{4}{c}{Grad} & \multicolumn{4}{c}{Int. Grad} \\
			\midrule
			 Atk. strategy & - & $\text{P-RGF}_D$ \cite{cheng2019improving} & EGTA & EGSA & EGSMA & $\text{P-RGF}_D$ \cite{cheng2019improving} & EGTA & EGSA & EGSMA & $\text{P-RGF}_D$ \cite{cheng2019improving} & EGTA & EGSA & EGSMA \\
			\midrule
			1k & 6.7 & 16.7& 26.7 & 17.7 & \bf 60.0 & 50.0 & \bf 76.7 &  10.0 & 53.3 & 20.0 &  \bf 23.3 & 6.7 & 11.7 \\
			\midrule
            4k & 10 & 23.3 & 26.7 & 27.1 & \bf 60.0 & 56.7 &  \bf 76.7 & 23.3 & 60.0 & \bf 23.3 & \bf 23.3 & 16.7 & 17.7 \\
            \midrule
            8k & 20 & 33.3 & 26.7 & 48.6 & \bf 66.7 & 67.7 & \bf 83.3 & 46.7 & 63.3 & 33.3 &  23.3 & 33.3 & \bf 53.3 \\
			\midrule
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption{Performance comparison on the soft-label attack success rate. Note that EGSA will give the same results for the true and absolute-valued explanations. $\text{P-RGF}_D$ \cite{cheng2019improving} uses various explanation as the prior, e.g, SmoothGrad. Notice that simply relies on the the transfer prior \cite{cheng2019improving} may lead to suboptimal attack due to the bias estimation of gradients.}
	\label{table:attack_succ_rate_s}
	\vspace{-1em}
\end{table*}

\begin{table*}[h]
	\centering
	\begin{adjustbox}{max width=0.8\textwidth}
		\begin{tabular}{c|c|c|ccc|ccc|ccc}
			\toprule
			% \multicolumn{2}{c}{Part}                   \\
			Atk. rate  & {None} & QEBA \cite{li2020qeba} & \multicolumn{3}{c}{Smooth Grad} & \multicolumn{3}{c}{Grad} & \multicolumn{3}{c}{Int. Grad} \\
			\midrule
			 Atk. strategy & - & - & EGTA & EGSA & EGSMA & EGTA & EGSA & EGSMA & EGTA & EGSA & EGSMA \\
             \midrule
             1k & 1.7 & 1.7 & \bf 68.8 & 1.7 & 5.1 & \bf 61.0 & 1.7 & 6.3 & \bf 23.8 & 1.7 & 3.4 \\
             \midrule
             4k & 5.1 & 6.8 & \bf 96.6 & 5.1 & 13.5 & \bf 98.3 & 8.5 & 12.0 & \bf 57.6 & 6.8 & 5.1 \\
			\midrule
            8k & 18.6 & 39.0 & \bf 98.3 & 32.2 & 54.2 & \bf 100 & 55.9 & 46.6 & \bf 76.3 & 32.2 & 33.9 \\
            \midrule
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption{Performance comparison on the hard-label attack success rate. QEBA \cite{li2020qeba} utilizes the gradient from 5 different surrogate models, such as ResNet-50, DenseNet-121, etc.}
	\label{table:attack_succ_rate_h}
	\vspace{-1em}
\end{table*}

% \begin{table}[h]
% 	\centering
% 	\begin{adjustbox}{max width=0.45\textwidth}
% 		\begin{tabular}{c|c|cc|cc|cc}
% 			\toprule
% 			% \multicolumn{2}{c}{Part}                   \\
% 			Atk. rate  & {None} & \multicolumn{2}{c}{Smooth Grad (true)} & \multicolumn{2}{c}{Grad (true)} & \multicolumn{2}{c}{Int. Grad (true)} \\
% 			\midrule
%             Attack strategy & - & $\text{P-RGF}_D$ \cite{cheng2019improving} & EGSMA & $\text{P-RGF}_D$ \cite{cheng2019improving} & EGSMA & $\text{P-RGF}_D$ \cite{cheng2019improving} &EGSMA \\
%             \midrule
%             1k & 6.7 & 16.7 & \bf 60.0 & 50 & \bf 53.3 & \bf 20.0 & 11.7 \\
%             \midrule
%             4k & 10 & 23.3 & \bf 60.0 & 56.7 & \bf 60.0 & \bf 23.3 & 17.7 \\
%             \midrule
%             8k & 20 & 33.3 & \bf 66.7 & \bf 67.7 & 63.3 & 33.3 & \bf 53.3 \\
% 			\midrule
% 			\bottomrule
% 		\end{tabular}
% 	\end{adjustbox}
% 	\caption{Performance comparison on the soft-label attack success rate for $L_2=1.25$. We compare with the previous state-of-the-art transfer-prior based attack where it uses the explanation as the prior. Notice that simply relies on the the transfer prior \cite{cheng2019improving} may lead to suboptimal attack due to the bias estimation of gradients.}
% 	\label{table:sota_prior}
% 	\vspace{-2.5em}
% \end{table}

% \begin{table}[h]
% 	\centering
% 	\begin{adjustbox}{max width=0.45\textwidth}
% 		\begin{tabular}{c|c|c|c|c|c}
% 			\toprule
% 			% \multicolumn{2}{c}{Part}                   \\
% 			Atk. rate  & {None} & QEBA \cite{li2020qeba} & Smooth Grad & Grad & Int. Grad \\
% 			\midrule
% 			Attack strategy & - & - & EGSMA & EGSMA & EGSMA \\ 
% 			\midrule
% 			1k & 1.7 & 1.7 & \bf 5.1 & 6.3 & 3.4 \\
% 			\midrule
% 			4k & 5.1 & 6.8 & \bf 13.5 & 12.0 & 5.1 \\
% 			\midrule
% 			8k & 18.6 & 39.0 & \bf 54.2 & 46.6 & 33.9 \\
% 			\bottomrule
% 		\end{tabular}
% 	\end{adjustbox}
% 	\caption{Performance comparison on the hard-label attack success rate for $L_2=12.5$. We compare with the previous state-of-the-art transfer-prior based attack where it utilizes the gradient from 5 different surrogate models, such as ResNet-50, DenseNet-121, etc.}
% 	\label{table:sota_prior_h}
% 	\vspace{-2.5em}
% \end{table}

Here we provide the following major guidelines to select different methods for different available explanations to perform EA based on the results:
\begin{itemize}
    \item For explanations that are close to the gradient, such as Smooth Grad and IntegratedGradients, it is recommended to apply EGTA to produce adversarial examples.
    \item For true explanations that are variants of the Gradient, including Guided Backprop and GradCam, the surrogate-model based attack EGSMA performs better. Besides, Table \ref{table:attack_succ_rate_s} and \ref{table:attack_succ_rate_h} show that EGSMA outperform the previous state-of-the-art transfer prior attack $\text{P-RGF}_D$ \cite{cheng2019improving} and QEBA \cite{li2020qeba}.
    \item For absolute-value explanations, the sampling-based attack EGSA can be applied to improve attack effectiveness. 
\end{itemize}

\subsection{Membership Inference Attack}
Here we construct the membership inference attack by measuring the accuracy of the membership inferenced by the attackers \cite{shokri2017membership, shokri2021privacy, yeom2018privacy} on 5 datasets: \textbf{CIFAR-10\cite{krizhevsky2009learning}}, \textbf{Purchases\cite{shokri2017membership}}, \textbf{Texas. \cite{shokri2017membership}}, \textbf{HAR\cite{li2021units, roggen2010collecting}}, and \textbf{Covid \cite{rahman_2021}}. Details about the datasets are provided in the appendix \ref{sec:dataset}.

\begin{table}[]
\begin{adjustbox}{max width=0.45\textwidth}
    \begin{tabular}{c|c|c|c|c}
    \toprule
    Works             & Ground-truth label & Probability prediction & Excessive queries & Explanation \\ \midrule
    \textit{MALT} \cite{sablayrolles2019white} &  \cmark      &      \cmark        &    \xmark       &   \xmark   \\ \midrule
    \textit{GAP-attack} \cite{yeom2018privacy}        &     \cmark      &      \xmark        &    \xmark       &   \xmark    \\ \midrule
    \textit{Boundary-attack} \cite{choquette2021label}  &     \cmark      &      \xmark        &    \cmark       &   \xmark       \\ \midrule
    \textit{OPT-var} \cite{shokri2021privacy}     &     \xmark      &      \xmark        &    \xmark       &   \cmark      \\ \midrule
    Ours       &     \xmark      &      \xmark        &    \xmark       &   \cmark      \\ \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{The requirements for performing MIA}\label{table:requirements}
\vspace{-2em}
\end{table}

\begin{table*}[h]
	\centering
	\begin{adjustbox}{max width=0.9\textwidth}
		\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
			\toprule
			% \multicolumn{2}{c}{Part}                   \\
% 			Accuracy & Sablayrolles et al. \cite{sablayrolles2019white} & Yeom et al. \cite{yeom2018privacy} & Christopher et al. \cite{choquette2021label} & Shokri et al.\cite{shokri2021privacy} & OPT-Grad. & OPT-Int. Grad & OPT-Smooth Grad  & OPT-GBP & OPT-GradCam & OPT-LIME\\
			Accuracy & \textit{MALT} \cite{sablayrolles2019white} & \textit{GAP-attack} \cite{yeom2018privacy} & \textit{Boundary-attack} \cite{choquette2021label} & \textit{OPT-var}\cite{shokri2021privacy} & OPT-Grad. & OPT-Int. Grad & OPT-Smooth Grad  & OPT-Guided Backprop & OPT-GradCam & OPT-LIME\\
            \midrule
            Covid & 69.0 & 55.7 & 64.0 & 51.8 & 66.8 & \bf 67.2 & 66.8 & 67.2 & 66.7 & 58.5 \\
            \midrule
            CIFAR-10 & 76.75 & 55.9 & 71.1 & 51 & 70 & 71.3 & 71.0 & 70.0 & 71.5 & \bf 73.8\\
            \midrule
            HAR & 60.0 & 56.2 & 56.8 & 48.9 & \bf 58.9 & 58.2 & 58.8 & 58.8 & 58.5 & - \\
            \midrule
            Purchase & 65.3 & 55.7 & 55.9 & 56.2 & 63.4 & \bf 63.7 & 63.5 & 63.4 & - & 62.3 \\
            \midrule
            Texas & 82.3 & \bf 77.8 & 77.1 & 64.2 & 73.0 & 72.2 & 71.5 & 73.0 & - & 76.0 \\ 
			\midrule
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption{Performance comparison on membership inference attack. Note that ours can achieve better accuracy than \textit{GAP-attack} \cite{yeom2018privacy} and \textit{Boundary-attack} \cite{choquette2021label}, and is comparable to \textit{MALT} \cite{sablayrolles2019white}, without additional attack access except explanations as shown in Table \ref{table:requirements}. Ours also outperform \textit{OPT-var}\cite{shokri2021privacy} using the same attack access.}
	\label{table:membership}
	\vspace{-2em}
\end{table*}

We randomly choose 8000 training samples from the private dataset and 8000 unseen samples for CIFAR-10, Purchase, and Texas. Due to the size of the training set of HAR and Covid, we choose 1000 private training samples and 1000 unseen samples. For each attack algorithm, the adversary also has 200 samples from the private training set to finetune the hyper-parameters of the attack algorithms. Table \ref{table:requirements} shows the required conditions to perform each attack, and Table \ref{table:membership} shows the results for membership inference attack using various attack methods:

% \textit{MALT} \cite{sablayrolles2019white} has shown that using loss as the indication of MIA is optimal given an optimal threshold under some assumptions and it becomes the upper bound of MIA. 

% \textit{GAP-attack} \cite{yeom2018privacy} predicts any misclassified data point as a non-member of the training set and vice versa. This is a naive baseline for label-only membership inference attack. The MIA prediction accuracy is equal to $50 + \frac{100-\text{Acc}}{2}$, where Acc is the classification accuracy on the test set. In this case, \textit{GAP-attack} \cite{yeom2018privacy} only works well on models that have a relatively lower classification accuracy, e.g., Texas dataset. 

% \textit{Boundary-attack} \cite{choquette2021label} uses the estimated distance to the decision boundary as an indication of membership. The attack works consistently well among all the datasets. However, we also need to point out that \textit{Boundary-attack} requires a harder condition to be performed as shown in Table \ref{table:requirements}. For instance, it needs access of the ground-truth label of a sample of interest. In some cases such as Covid-19 pneumonia data \cite{rahman_2021}, this may rely on the expert's domain knowledge and be expensive to obtain. Besides, it also requires thousands time more queries to estimate decision boundary much may renders a costly attack. 

% \textit{OPT-var} \cite{shokri2021privacy} is not a strong indication for Covid, CIFAR-10, and HAR datasets but informative for Purchase and Texas datasets as reported.

\textit{MALT} \cite{sablayrolles2019white} has shown that using loss as the indication of MIA is optimal given an optimal threshold under some assumptions, and it becomes the upper bound of MIA. \textit{GAP-attack} \cite{yeom2018privacy} predicts any misclassified data point as a non-member of the training set and vice versa. This is a naive baseline for label-only membership inference attacks. \textit{GAP-attack} only works well on models that have a relatively lower classification accuracy, e.g., Texas dataset. \textit{Boundary-attack} \cite{choquette2021label} uses the estimated distance to the decision boundary as an indication of membership. The attack works consistently well among all the datasets. However, we also need to point out that \textit{Boundary-attack} requires a harder condition to be performed, as shown in Table \ref{table:requirements}. It needs access to the ground-truth label of a sample of interest and requires thousands of more queries to estimate decision boundary, which may render a costly attack. As is reported in \cite{shokri2021privacy}, \textit{OPT-var} is not a strong indication for Covid, CIFAR-10, and HAR datasets but informative for Purchase and Texas datasets.

After revisiting the relation between explanations and MIA, we found that explanations actually carry much richer membership information instead of what is claimed by \textit{OPT-var} \cite{shokri2021privacy}. Here we define the advantage as $p_{\text{acc}} - p_{\text{rand}} = p_{\text{acc}} - 50$, i.e., the improvement of accuracy over random guess 50\%, and we observe a significant increase compared to the previous \textit{OPT-var}. For instance, OPT-Grad outperforms \textit{OPT-var} consistently by more than 100\%. Besides, Smooth Grad, which is treated as perturbation-based explanation methods and criticized for not following the distribution of the training data \cite{shokri2021privacy}, performs constantly well as other gradient-based explanations. This indicates that Smooth Grad is also authentic to the model, and the membership information is also maintained by such explanations. Furthermore, even region-based explanation Grad-Cam also contains informative membership information. Lastly, in contrast to the claim in \cite{shokri2021privacy} that LIME explanation does not perform better than a random guess, the LIME explanations outperform many other approaches and result in meaningful membership indications. Please note that GradCam cannot be applied naturally to Purchase and Texas because the trained neural networks only consist of a fully connected layer and do not use multiple channels and pooling operations. Besides, we also omitted to apply LIME to time-series data because LIME cannot be naturally extended to this modality.

\subsection{Model Extraction attack (MEA)}
Here we show the results of MEA on 4 different datasets: CIFAR-10, MNIST~\cite{deng2012mnist}, Covid, and HAR. The first threes are on the image domain, and HAR is time-series data. Following \cite{tramer2016stealing}, we plot the test mismatch on the test dataset as the followings:
\begin{equation}
    R_{\text{test}} = T_{\text{test}} - \hat{T}_{\text{test}}
\end{equation}
where $\hat{T}_{\text{test}}$ is the test accuracy of the extracted model $\hat{F}(\boldsymbol x)$ obtained using simple prediction matching or the explanation matching. $T_{\text{test}}$ is the test accuracy of the victim model $F(\boldsymbol x)$ on the test dataset. $R_{\text{test}}$ is the measure of how effective the MEA mechanism is to produce a model with equivalent task accuracy, \revisionPQ{}{which works as a proxy for \textit{functionally equivalent}.}


\begin{figure}[h]
    \minipage{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/MEA/CIFAR10_False_.eps} (a) CIFAR-10 \centering \par
    \endminipage\hfill
    \minipage{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/MEA/MNIST_False_.eps}  (b) MNIST \centering \par
    \endminipage\hfill
    
    \minipage{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/MEA/Covid_False_.eps} (c) Covid \centering  \par
    \endminipage\hfill
    \minipage{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/MEA/HAR_False_.eps} (d) HAR \centering \par
    \endminipage\hfill

		\caption{$R_{\text{test}}$ on various dataset. We show the performance of 6 various explanations and the baseline (without explanations).}
	\label{fig:MEA-cifar10}
% 	\vspace{-.5em}
\end{figure}

\subsubsection{MEA results}

Fig. \ref{fig:MEA-cifar10} (a) shows $R_{\text{test}}$ with respect to various of query budgets and explanation mechanisms on CIFAR-10 dataset. First, we can observe that with the help of the explanation matching mechanism, the adversary can have the advantage of producing an extracted model with higher accuracy. For instance, to produce an extracted model with 25 test mismatches, the without-explanation baseline consumes $10^4$ queries, while the Gradient and Guided Backprop gradient matching mechanism can have an 84\% query reduction. In this case, to perform the MEA attack on Machine learning as a service (MLaaS) using query API, the monetary costs are at $\approx$\$0.25 per query. \footnote{\url{https://www.clarifai.com/pricing}} Then, using the explanation-matching mechanism can reduce the cost by \$2100.

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/MEA/MNIST_False_.eps} \par
%     \endminipage\hfill
%     \vspace{-0.5em}
% 		\caption{$R_{\text{test}}$ on MNIST dataset}
% 	\label{fig:MEA-mnist}
% % 	\vspace{-.5em}
% \end{figure}

For the MNIST dataset, we can also have a similar observation where explanations of various forms can help reduce the test mismatch $R_{\text{test}}$ in Fig. \ref{fig:MEA-cifar10} (b). Among them, LIME, Guided Backprop, and Smooth Grad have the highest improvement using various query budgets. For instance, LIME can produce a task-accuracy equivalent model using $10^3$ queries, which has about 90\% costs reduction compared to the without-explanation baseline.

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/MEA/Covid_False_.eps} \centering  \par
%     \endminipage\hfill
%     \vspace{-0.5em}
% 		\caption{$R_{\text{test}}$ on Covid dataset}
% 	\label{fig:MEA-covid}
% % 	\vspace{-.5em}
% \end{figure}

For the Covid dataset, the improvement is highly modest, as shown in Fig. \ref{fig:MEA-cifar10} (c). The baseline approach has about $R_{\text{test}}=40$. And most of the explanation-matching schemes fluctuate around the baseline with various query budgets. We also note that Gradient, LIME, and Guided Backprop have a clear increase in test mismatch, i.e., using the explanation-matching mechanism decreases the MEA performance. However, one clear exception is GradCam. Using 2000 queries, GradCam reduces $R_{\text{test}}$ from 42 to 30, where it shows around 25\% improvement.

% \begin{figure}[h]
%     \minipage{0.45\textwidth}
%         \includegraphics[width=\linewidth]{images/MEA/HAR_False_.eps} \centering \par
%     \endminipage\hfill
%     \vspace{-0.5em}
% 		\caption{$R_{\text{test}}$ on HAR dataset}
% 	\label{fig:MEA-har}
% % 	\vspace{-.5em}
% \end{figure}

Fig. \ref{fig:MEA-cifar10} (d) shows the MEA results on the HAR dataset. Similarly, we can observe that matching explanations do not improve the MEA performance using various queries in most cases. The only exception is GradCam, where the performance improves marginally. 

\subsubsection{Mean-Square-Value (MSV) of explanations as a strong indication}
Here we further investigate the reason why explanation matching has a clear improvement on the CIFAR-10 and MNIST dataset, while the improvement is relatively modest on the other two. Here we plot the Mean-Square-Value (MSV) with each explanation:

\begin{equation}
    MSV = \frac{1}{n} \sum_{i=1}^{n}E_i^2
\end{equation}

where $E \in \mathbb{R}^n$ is the explanation generated by the model. The MSV calculated the $L_2$-norm of $E$ normalized by its dimension. Table. \ref{table:MSV} shows the averaged MSV of different explanations of 1000 samples from each dataset. We can observe from Table. \ref{table:MSV} that the MSV has a strong correlation with the improvement made by each explanation method: a higher MSV can produce a larger advantage of performing MEA. We omit the value of LIME here since we does not rely on explanation matching but prediction matching to perform MEA.

First, the values of MSV of HAR and Covid are orders of magnitude smaller than those of CIFAR-10 and MNIST, which means that the explanations of HAR and Covid have limited information to be extracted. And matching the explanations does not produce a clear improvement in the performance of MEA. The relatively small gradient is caused by the overfitting of the model in the two datasets because instances from the training distribution will cause a small loss for the model and render a smaller gradient. On the other hand, the MSVs of explanations in the CIFAR-10 and MNIST datasets are consistently large, and we observe a more significant improvement of MEA. Besides, we also notice that the MSV of GradCam is consistently larger among all the datasets. And we notice a clear improvement in the attack performance produced by explanation matching using GradCam, which is in line with a larger MSV of GradCam.

\begin{table}[h]
	\centering
	\begin{adjustbox}{max width=0.43\textwidth}
		\begin{tabular}{c|c|c|c|c|c}
			\toprule
            Dataset & Grad & Int. Grad & Smooth Grad & Grad-Cam & Guided Backprop\\
            \midrule
            CIFAR-10 & 7.4e-1 & 7.8e-2 & 5.1e-1 & 5.2e-1 & 7.1e-1 \\
            \midrule
            MNIST & 7.5e-2 & 3.4e-2 & 7.3e-2 & 7.2e-2 & 7.4e-2 \\
            \midrule
            HAR & 7.0e-10 & 2.1e-4 & 7.0e-10 & 2.1e-1 & 7.8e-10 \\
            \midrule
            Covid & 2.2e-3 & 2.0e-3 & 9.0e-4 & 4.7e-2 & 1.5e-5\\
			\midrule
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption{Mean-Square-Value (MSV) of each explanation. The value is averaged over 1000 samples.}
	\label{table:MSV}
	\vspace{-3em}
\end{table}

==> TIFS-2022 (Arxiv) 2/intro.tex <==
\section{Introduction}
\label{sec:intro}

% % In recent years, there has been an surge in the development and application of deep models, yielding varying degrees of success across a broad range of tasks. Many of them are security-critical such as content moderation~\cite{ccitlak2019survey}, spam filtering~\cite{wu2018twitter}, autonomous driving~\cite{huang2020autonomous}, healthcare~\cite{tonekaboni2019clinicians} and criminal justice~\cite{zavrvsnik2020criminal}. Despite these remarkable achievements, however, deep learning algorithms have proven to be brittle against security and privacy attack, e.g., Evasion Attack (EA): generating adversarial that are perceptually indistinguishable from the input but are designed to cause targeted or untargeted misclassification to evade detection \cite{goodfellow2014explaining}. Therefore, the popularity of deep models has led to an increase concern of the potential security and privacy risks.

% In recent years, the interpretability and the transparency of the adoption of deep models is required to build trustworthy and reliable deep learning systems, which will otherwise be black-box and opaque ~\cite{tonekaboni2019clinicians,vellido2019importance}. The interpretability of deep models are believed to ensure models' reliability and fairness and also prevent the potential risks, which is increasingly required by laws. For instance, data regulatory policies, such as EU's GDPR\footnote{\url{https://gdpr-info.eu/}} states it an individual has a right to an \emph{explanation} for decisions that significantly affect the individual ('Right to Explanation'). Thus, deployed models are continually required to output both their decision as well as an explanation of the decision. These post-hoc explanations are usually presented in the form of a saliency map over the input, highlighting features that were the most relevant to the model decision. 

% However, these post-hoc explanations, as they leak information about the black-box model's internal decision process, may serve as an information-rich side-channel, available to an adversary in addition to the model output, and develop efficient and effective attack. For instance, \cite{shokri2021privacy, milli2019model} has shown that explanations can leak private information about the model and the attribution of data. However, the previous works have not studied the connection between post-hoc explanations and the evasion attacks. Besides, there are still lacking an in depth study of the risks produced by common explanations and providing a guideline for system developers to choose a secure explanation mechanism. In this work, we try to fill the aforementioned gap. 

% \begin{table}[]
% \begin{adjustbox}{max width=0.40\textwidth}
%     \begin{tabular}{c|c}
%     \hline
%     Explanation & criterion\\ 
%     \hline
%     Gradient~\cite{simonyan2013deep} & Fidelity~\cite{yeh2019fidelity}, ROAR~\cite{adebayo2018sanity}\\
%     \hline
%     Guided-backprop~\cite{springenberg2014striving} & ROAR~\cite{adebayo2018sanity}\\
%     \hline
%     Smooth Grad~\cite{smilkov2017smoothgrad} & Fidelity~\cite{yeh2019fidelity}\\
%     \hline
%     Int. Grad~\cite{sundararajan2017axiomatic} & Fidelity~\cite{yeh2019fidelity}\\
%     \hline
%     Grad-Cam~\cite{selvaraju2017grad} & User study~\cite{jeyakumar2020can}\\
%     \hline
%     LIME~\cite{ribeiro2016should} & User study~\cite{jeyakumar2020can}\\
%     \hline
%     \end{tabular}
% \end{adjustbox}
% \caption{The selection of explanations}\label{table:criteria}
% \vspace{-2em}
% \end{table}

% Table \ref{table:criteria} identifies 6 popular and widely-used explanations according to established criteria in the literature. \textit{Fidelity}~\cite{yeh2019fidelity} focuses on the closeness of the predictions between the true model and the linear model approximated by the explanations. \textit{ROAR}~\cite{adebayo2018sanity} defines the sensitivity of the explanation methods to the randomization of the inputs. \textit{User study}~\cite{jeyakumar2020can} shows which style
% of explanation is preferred by end-users. Based on the explanation methods of interest, we explore the use of the above explanations as a side-channel for an adversary to develop efficient evasion attack (EA), membership inference attack (MIA), and model extraction attack (MEA).

% Regarding EA for most real-world systems, adversarial examples need be generated in a constrained \emph{black-box setting}, in which an adversary can only repeatedly querying the target model for its prediction~\cite{ilyas2018black, chen2017zoo}. But, the costs associated with queries can render a query-inefficient black-box attack impractical~\cite{ilyas2018black}. Towards this end, we propose three novel attack schemes for query reduction: Explanation-Guided Transfer Attack (EGTA), Explanation-Guided Surrogate Model Attack (EGSMA), and Explanation-Guided Sampling Attack (EGSA). (\romannumeral 1) EGTA directly use the explanation as the transfer prior to shape a search distribution for estimating the gradient~\cite{ilyas2018black}, which is applicable when the explanation has high cosine similarity to the true gradient; (\romannumeral 2) On the other hand, if the explanation has low cosine similarity, the direct use of the explanation may lead to large bias of gradient estimation. We thus propose EGSMA to use a surrogate model to mimic the behavior of the victim model (that is being attacked) and uses explanation to train the surrogate model. (\romannumeral 3) Furthermore, when the absolute values of the explanation is returned as proposed in previous literature \cite{smilkov2017smoothgrad, sundararajan2017axiomatic}, we further come up with EGSA to incorporate the prior explanations by shaping the covariance matrix of the search distribution.

% Second, we revisit the membership information leaked by common explanations, where the adversary can exploit model explanations to infer whether a data belongs to the training set of a model. Here we propose to use the variance of explanation produced from the softmax score of the output as the indication of membership. Instead of claiming by the previous works \cite{shokri2021privacy} that the advantages are limited for common explanations, we observe leakage of a significant amount of information about individual membership. 

% Finally, we also study advantages of amounting Model Extraction Attack (MEA) using various explanations. The goal of the adversary is to extract a black-box model by only querying the model prediction. We connect the advantages of MEA using explanations to the mean square values of explanations.

% In summary, we make the following contributions:
% \vspace{-1em}
% \begin{itemize}
%     \item We exploit explanations as a side-channel and develop explanation-guided black box evasion attacks. We show a $10\times$ query budget reduction when a gradient-based explanation is available.
%     \item We also theoretically characterize the advantage of the proposed explanation-guided evasion attack using a total variance reduction prospective.
%     \item We revisit the membership information leaked by common explanations and observe leakage of a significant amount of information about individual membership by explanations.
%     \item We empirically study advantages of amounting Model Extraction Attack (MEA) using various explanations and connect the advantages of MEA to the mean square values of explanations.
%     %and propose a reasonable range for adding DP-noise that maintains high utility and strong privacy.
% \end{itemize}



% % \section{Introduction}
% % \label{sec:intro}
% % One of the main tenets of trustworthy AI is decisional transparency of deep learning models~\cite{tonekaboni2019clinicians,vellido2019importance}. Data regulatory policies, such as EU's GDPR\footnote{\url{https://gdpr-info.eu/}} states it an individual has a right to an \emph{explanation} for decisions that significantly affect the individual ('Right to Explanation'). Thus, deployed models are increasingly required to output both their decision as well as an explanation of the decision. These post-hoc explanations are usually presented in the form of a saliency map over the input, highlighting features that were the most relevant to the model decision. 

% % At the same time, there has been an increase in the adoption of deep models for security-critical tasks such as content moderation~\cite{ccitlak2019survey}, spam filtering~\cite{wu2018twitter}, autonomous driving~\cite{huang2020autonomous}, healthcare~\cite{tonekaboni2019clinicians} and criminal justice~\cite{zavrvsnik2020criminal}. The application of deep models has led to an increase in adversarial examples: specially crafted data samples that are perceptually indistinguishable from the input but are designed to cause targeted or untargeted misclassification to evade detection or achieve some other adversarial objectives~\cite{goodfellow2014explaining}. Several successful strategies have been proposed for generating adversarial examples in the \emph{white-box setting}, where the adversary is assumed to have access to both the model weights and can also compute the gradients~\cite{art}. For most real-world systems, however, adversarial examples must be generated in a more constrained \emph{black-box setting}, in which an adversary does not have access to the model weights and cannot compute the gradients. These black-box attacks operate by repeatedly querying the target model and using the responses to estimate the gradient direction in which to perturb the input~\cite{ilyas2018black, chen2017zoo}. But, the costs associated with queries, limits on the maximum number of daily queries, or the risk of detection due to a high number of similar queries, can render a query-inefficient black-box attack impractical~\cite{ilyas2018black}. 

% % In this work, we explore the use of explanations as an information-rich side-channel, available to an adversary in addition to the model output, and develop query-efficient black-box attacks. We focus on the class of post-hoc explanation mechanisms (such as Gradient~\cite{goodfellow2014explaining}, Integrated Gradients~\cite{sundararajan2017axiomatic}, and SmoothGrad~\cite{smilkov2017smoothgrad}) that use gradient information to generate saliency maps over the input space. We posit that through careful adversarial manipulation the information in the explanation can be used to perform more accurate gradient estimation with a fewer number of queries. 

% % Towards this end, we propose three novel attack schemes: Explanation-Guided Transfer Attack (EGTA), Explanation-Guided Sampling Attack (EGSA) and Explanation-Guided Surrogate Model Attack (EGSMA). These attacks (both targeted and untargeted) exploit the explanation in different ways to improve gradient estimation accuracy. EGTA and EGSA use the explanation to shape a search distribution that is often used for estimating the gradient~\cite{ilyas2018black}. EGSMA uses a surrogate model to mimic the behavior of the victim model (that is being attacked) and uses explanation to train the surrogate model. To assess the performance of the attacks, we consider two different threat models. We consider a \emph{Hard-label} setting, where only the model decision along with the explanation is available to the adversary. This is the most restrictive black-box setting.  We then consider a \emph{Soft-label} setting, in which the predicted probabilities over all the classes are available with the explanation. We demonstrate using several benchmarking datasets and models, our attacks perform well under these highly restrictive but practical threat models and significantly improve upon query efficiency. 

% % Finally, we discuss mitigation approaches and in particular, propose a differential privacy (DP)-based mechanism \cite{dwork2006differential} to intercept the gradient vector and make it differentially private before releasing it to the explanation mechanisms. We show that our DP-based mechanism can be used to guarantee the indistinguishability of gradient vectors. This in turn makes it difficult to use explanations for gradient estimation minimizing the adversarial advantage. We observe that there is a tradeoff between the magnitude of noise added to reduce adversarial advantage and the utility of the explanation to the end-user. We use several metrics to quantify the subjective utility of an explanation and its variation with the level of differential privacy chosen.

% % In summary, we make the following contributions:
% % \begin{itemize}
% %     \item We exploit explanations as a side-channel and develop explanation-guided black box attacks. We show a $10\times$ query budget reduction when true gradient-based explanation is available (EGTA) in the hard-label setting and a $2\times$ query reduction when the absolute-value of the gradient is used for generating explanation (EGSA) in the soft-label setting.
% %     \item We propose a surrogate model-based learning framework (EGSMA), that achieves $100.4\%$ higher attack success rate than attacks directly using explanation to shape the search distribution, and is $133.5\%$ higher than the previous black-box attacks~\cite{ilyas2018black}.
% %     \item We propose a differential privacy (DP)-based provable defense to minimize the risk of providing explanations. We show that explanations, output by the gradient-based explanation mechanisms, are also differentially private. 
% %     \item We empirically demonstrate the risk of bypassing DP-based defense using an adaptive attack based on averaging multiple explanations. We evaluate and study the trade-off between utility and privacy of explanations.
% %     %and propose a reasonable range for adding DP-noise that maintains high utility and strong privacy.
% % \end{itemize}

Post-hoc explanations~\cite{simonyan2013deep, springenberg2014striving, smilkov2017smoothgrad, sundararajan2017axiomatic} have emerged as the primary means of introducing decisional transparency into deep neural networks-based systems, which are otherwise complex and operate as opaque black-boxes. These explanations are usually presented to the user in the form of a saliency map over the input, highlighting features that were the most relevant to the model decision. Thus, deployed models output both their decision as well as the explanation of the decision to ensure reliability~\cite{tonekaboni2019clinicians}, fairness~\cite{anders2020fairwashing}, and compliance to data regulatory policies \footnote{\url{https://gdpr-info.eu/}}.

However, as these post-hoc explanations are derived using information from the model's parameters and gradients, they also serve as an information-rich side-channel that is available to an adversary, in addition to the model decision. For instance, ~\cite{shokri2021privacy, milli2019model} have shown that explanations can leak private information about both the model and data attributes. \revisionPQ{}{In this paper, we perform a systematic characterization of the privacy and security risks, quantified by \emph{increased efficiency} (e.g., reduced query count, attack feasibility in constrained settings and so on) of evasion attacks (EA), membership inference attacks (MIA) and model extraction attacks (MEA), due to the release of explanations.}

%Para on Evasion Attacks
We consider evasion attacks on real-world systems, which are usually mounted in a \emph{black-box setting}. An adversary (with no access to the model parameters and gradients) repeatedly queries the victim model (that is being attacked) to design adversarial examples, eliciting targeted misclassification~\cite{ilyas2018black, chen2017zoo}. However, the cumulative costs associated with a large number of queries can render a query-inefficient black-box attack impractical~\cite{ilyas2018black}. Towards this end, we propose three novel explanation-guided evasion attacks, that significantly reduce the number of queries needed, making these attacks highly feasible in practice. In (\romannumeral 1) Explanation-Guided Transfer Attack (EGTA), we directly use  explanations as a transfer prior to shape a search distribution for estimating the gradient~\cite{ilyas2018black}. This attack is highly efficient when the estimated gradient (using explanations) has high cosine similarity to the true gradient; (\romannumeral 2) If the cosine similarity is low, using the explanation as a prior leads to a highly biased gradient estimation. The Explanation-Guided Surrogate Model Attack (EGSMA), instead uses explanations to train a surrogate model and mimic the decisions of the victim model. Gradient from the surrogate model is then used to generate the adversarial examples. (\romannumeral 3) Finally, when absolute value of the true gradients is used to generate explanations~\cite{smilkov2017smoothgrad, sundararajan2017axiomatic}, we propose to use the Explanation-Guided Sampling Attack (EGSA). In this, we use explanations to shape the covariance matrix of the search distribution, used to estimate the gradients. Finally, we show that the adversarial advantage due to explanations can be quantified as a reduction in the total variance of the estimated gradients.

%Para on Membership Inference
We then revisit the problem of membership information leaked by explanations. In this, the goal of an adversary is to exploit model explanations to infer the membership of a sample in the training data. We build on the intuition provided in prior work that variance in explanations can be used as an indicator of membership, in black-box settings~\cite{shokri2021privacy}. However, we use the softmax score of the output, as opposed to the logit layer score (as proposed earlier) to generate the explanation and compute the variance. Contrary to the observations in \cite{shokri2021privacy}, using our modified attack, we found significant leakage of membership information via explanations.

Finally, we study the adversarial advantage due to explanations in mounting model extraction attacks. The goal of the adversary is to train a surrogate model that is \emph{functionally equivalent} to the victim model in a black-box setting. We demonstrate significant query reduction and also connect the adversarial gain to the mean square values (MSV) of explanations: a higher MSV results in a larger adversarial advantage in performing MEA. 

\noindent{\bf Choice of Explanation Techniques:} To determine a representative subset of explanation techniques, we use three metrics: (i) \textit{Fidelity}~\cite{yeh2019fidelity} which focuses on the closeness of the predictions between the true model and the linear model approximated by the explanations given random input perturbation; (ii) \textit{ROAR}~\cite{hooker2019benchmark} computes the change in model accuracy after removing the important features and retraining; (iii) \textit{User study}~\cite{jeyakumar2020can} identifies explanation types that are preferred by end-users. These can differ based on the modality of the data that are used to evaluate and rank explanations. Accordingly after a survey of various papers, we selected six explanation techniques (Table \ref{table:criteria}) which ranked highly as per the above metrics.

\begin{table}[]
\centering
\begin{adjustbox}{max width=0.40\textwidth}

    \begin{tabular}{l|l}
    \hline
    Explanation & criterion\\ 
    \hline
    Gradient~\cite{simonyan2013deep} & Fidelity~\cite{yeh2019fidelity}, ROAR~\cite{hooker2019benchmark}\\
    \hline
    Guided backprop~\cite{springenberg2014striving} & ROAR~\cite{hooker2019benchmark}\\
    \hline
    Smooth Grad~\cite{smilkov2017smoothgrad} & Fidelity~\cite{yeh2019fidelity}\\
    \hline
    Int. Grad~\cite{sundararajan2017axiomatic} & Fidelity~\cite{yeh2019fidelity}\\
    \hline
    Grad-Cam~\cite{selvaraju2017grad} & User study~\cite{jeyakumar2020can}\\
    \hline
    LIME~\cite{ribeiro2016should} & User study~\cite{jeyakumar2020can}\\
    \hline
    \end{tabular}
\end{adjustbox}
\caption{Explanations and their corresponding metrics}\label{table:criteria}
\vspace{-2em}
\end{table}

In summary, we make the following contributions:

\begin{itemize}
    \item We exploit explanations as a side-channel and develop explanation-guided black box evasion attacks. We show a $10\times$ reduction in query count when a gradient-based explanation is available. We provide theoretical analysis of the adversarial gain and quantify it as the reduction in variance of the gradient estimate.
    
    \item We propose a modified attack for extracting membership information from explanations and report significant leakage compared to prior work.
    
    \item We demonstrate large query reduction for model extraction attack using explanations.
\end{itemize}

==> TIFS-2022 (Arxiv) 2/related.tex <==
\section{Related Work}
\label{sec:related}
We group prior work into two categories: (i) Post-hoc explanation mechanisms; and (ii) The intersection of explanation and security and privacy risks.\\

\noindent{\bf Post-hoc explanation mechanisms:} These are after-the-prediction explanation mechanisms that aim to provide evidence to elucidate the model decision~\cite{expl_survey,jeyakumar2020can}. Post-hoc explanation techniques are broadly divided into (i) textual explanations of system outputs, (ii) visualisations of learned representations or models (e.g., saliency maps), and (iii) explanations-by-example~\cite{jeyakumar2020can}. In our work, we focus on (ii) post-hoc mechanisms that generate saliency maps, and describe them briefly as follows.

\begin{itemize}[leftmargin=*]
\item Gradient-based saliency map: GradientInput~\cite{simonyan2013deep}, IntegratedGradient~\cite{sundararajan2017axiomatic}, GradCam~\cite{selvaraju2017grad}, and SmoothGrad~\cite{smilkov2017smoothgrad} visually highlight the feature components that has large affects on the model prediction using gradient-based techniques.
\item Local interpretable surrogate model: LIME~\cite{ribeiro2016should} transforms a black-box model into a transparent one by training a surrogate interpretable model on the point of interests.

\end{itemize}
% \begin{itemize}[leftmargin=*]
% \item GradientInput~\cite{simonyan2013deep}: Generates the saliency by computing the (signed) partial derivative of the model output with respect to the input and then multiplying it element-wise with the input features.

% \item IntegratedGradient~\cite{sundararajan2017axiomatic}: Computes the average over gradients from a set of scaled images followed by element-wise product with the original image. Specifically, integrated gradients are defined as the path integral of the gradients along a straight line from the baseline to the input.
 
% \item SmoothGrad~\cite{smilkov2017smoothgrad}: Helps visually sharpen gradient-based sensitivity maps. This technique adds pixel-wise Gaussian noise to many copies of the image, and then it averages the resulting gradients to generate the saliency map.

% \item GradCam~\cite{selvaraju2017grad}: Uses the gradients of any target concept, e.g., logit of a class, flowing into the final convolutional layer to produce a coarse localization map highlighting the important regions in the data space.

% \item GuidedBackprop~\cite{springenberg2014striving}: Computes the gradient of the target output with respect to the input, but gradients of ReLU functions are overridden so that only non-negative gradients are backpropagated.

% \item LIME~\cite{ribeiro2016should}: Transforms a black-box model into a transparent one by training a surrogate interpretable model on the point of interests, which enjoys the flexibility of explaining different models in various modalities.

% \item GradientSHAP~\cite{lundberg2017unified}: Calculates SHAP scores that are based on the Shapley values proposed in cooperative game theory. Gradient SHAP combines ideas from IntergratedGradient and SmoothGrad where it adds Gaussian noise multiple times to each input set, chooses a random point along the path between baseline and input, and computes the gradient of outputs with respect to those random points. The expected value is used as the final SHAP score.
% \end{itemize}

\medskip
\noindent{\bf Model Explanations and Adversarial Attacks:} Complementary to our work, there has been several recent papers that have explored the connection between adversarial attacks and explanations. 

\begin{itemize}[leftmargin=*]
% \item Explanation-Guided Poisoning Attack: The authors in~\cite{shap_poisoning} have used SHapley Additive Explanations (SHAP) to identify features in the input samples that should be perturbed/poisoned to insert a backdoor trigger into the model during training. In contrast, we use explanation for gradient estimation and generate adversarial examples.

\item Explanation-Guided Membership Inference Attack: \cite{shokri2021privacy} has shown that an adversary can exploit model explanations to infer whether a data belongs to the training set of a model, i.e., mounting Membership Inference Attack (MIA).

\item Explanation-Guided Model extraction Attack: Besides, \cite{milli2019model} demonstrate that gradient-based explanations of a model can help the adversary to perform efficient Model Extraction Attack (MEA), i.e., copying the model without authorization, contradicting the intention of keep a proprietary model secret.

% \item Attacks on Explanations and Robustness: Prior work has explored the robustness of explanation in adversarial settings in which the explanation itself was attacked. \cite{ghorbani2019interpretation, basu2020influence, levine2019certifiably} observed that the output of commonly used explanation methods can be changed drastically using imperceptible perturbation in the inputs. The attack indicates the need to build reliable explanation methods.
\end{itemize}
Orthogonal to our study, there was also been work on attacking explanations for various objectives such as reducing trust on the model decision~\cite{iccv_fooling} and fairwashing~\cite{anders2020fairwashing}.

However, none of the above study how explanations can benefit evasion attacks. Besides, there has not been a systematic study on the security and privacy risk for popular explanations types. Therefore, this work aims at filling the aforementioned gaps.


